A Review of BioTree Construction in the Context of Information Fusion: Priors, Methods, Applications and Trends

Biological tree (BioTree) analysis is a foundational tool in biology, enabling the exploration of evolutionary and differentiation relationships among organisms, genes, and cells. Traditional tree construction methods, while instrumental in early research, face significant challenges in handling the growing complexity and scale of modern biological data, particularly in integrating multimodal datasets. Advances in deep learning (DL) offer transformative opportunities by enabling the fusion of biological prior knowledge with data-driven models. These approaches address key limitations of traditional methods, facilitating the construction of more accurate and interpretable BioTrees. This review highlights critical biological priors essential for phylogenetic and differentiation tree analyses and explores strategies for integrating these priors into DL models to enhance accuracy and interpretability. Additionally, the review systematically examines commonly used data modalities and databases, offering a valuable resource for developing and evaluating multimodal fusion models. Traditional tree construction methods are critically assessed, focusing on their biological assumptions, technical limitations, and scalability issues. Recent advancements in DL-based tree generation methods are reviewed, emphasizing their innovative approaches to multimodal integration and prior knowledge incorporation. Finally, the review discusses diverse applications of BioTrees in various biological disciplines, from phylogenetics to developmental biology, and outlines future trends in leveraging DL to advance BioTree research. By addressing the challenges of data complexity and prior knowledge integration, this review aims to inspire interdisciplinary innovation at the intersection of biology and DL.

==> macros.tex <==
\def\weight{w}
\def\mweight{\theta}
\def\pweight{\phi}


\newcommand{\policy}{\pi}
\def\Ob{\bm{O}}
\def\ob{o}
\def\Ac{\va}
\def\ac{a}
\def\St{\vs}
\def\st{s}
\def\lat{\vz}
\def\rew{r}
\def\Rew{R}
\def\Val{V}
\def\Qval{Q}
\def\df{\gamma}
\def\pol{\pi}
\def\rlt{\xi}
\def\history{\rlt}
\def\eplen{H}
\def\samplinghorizon{\mathcal{h}}
\def\trans{\gT}
\def\hidden{h}
\def\meta{m}
\def\conv{\texttt{conv}}
\def\rnn{\texttt{rnn}}
\def\lstm{\texttt{lstm}}


\def\bid{\vq}
\def\bidd{q}
\def\price{\vp}
\def\pricee{p}
\def\wealth{w}
\def\Wealth{W}
\def\util{u}
\def\Util{U}
\def\utility{\util}
\def\Utility{\Util}

\def\endow{x}
\def\vendow{\V{\endow}}
\def\margendow{dx}
\def\vmargendow{\V{\margendow}}
\def\initendow{\endow_0}

\newcommand{\posttax}[1]{\tilde{#1}}

\def\skill{n}
\def\type{\theta}
\def\elas{e}
\def\elasticity{\elas}

\def\income{z}
\def\consumption{c}
\def\capital{k}
\def\production{y}

\def\effort{Q}
\def\labor{l}
\def\vlabor{\V{\labor}}

\def\crra{\texttt{crra}}
\def\laborcoeff{c}
\def\isoeta{\eta}

\def\tax{T}
\def\taxrate{\tau}
\def\mtaxrate{\tau}
\def\taxperiodlen{M}

\def\bracketcutoff{m}

\def\tradetax{ {T_{\textrm{trade}}} }
\def\vtradetax{ {\V{\tradetax}} }
\def\tradetaxrate{ {\tau_{\textrm{trade}}} }

\def\wealthtax{ {T_{\vendow}} }
\def\vwealthtax{ {\V{\wealthtax}} }
\def\wealthtaxrate{ {\tau_{\vendow}} }

\def\incometax{ T }  %
\def\vincometax{ {\V{\incometax}} }
\def\incometaxrate{ {\tau_{\income}} }

\def\incomesubsidy{ {\tau_{\income}} }

\def\money{\endow^c}
\def\posttaxmoney{\posttax{\endow}^c}
\def\paretoinputmoney{\income}

\def\stone{\endow^s}
\def\wood{\endow^w}
\def\house{\endow^h}

\def\Money{\vendow^c}

\newcommand{\mon}[2]{\money_{#1,#2}}
\newcommand{\sto}[2]{\stone_{#1,#2}}
\newcommand{\woo}[2]{\wood_{#1,#2}}
\newcommand{\hou}[2]{\house_{#1,#2}}


\def\pdf{f}
\def\cdf{F}
\def\gini{\texttt{gini}}
\def\equality{\texttt{eq}}
\def\productivity{\texttt{prod}}


\def\socialplanner{\pi_p}
\def\plannerpolicy{\pi_p}
\def\socialwelfare{\texttt{swf}}
\def\SWF{\socialwelfare}
\def\socialwelfareweight{\omega}
\def\paretoweight{g}
\def\socialmarginalwelfareweight{\paretoweight}
\def\camelback{"Camelback"}


\newcommand{\idxtime}[2]{{#1}_{#2}}
\newcommand{\idxagent}[2]{{#1}_{#2}}
\newcommand{\idxgood}[2]{{#1}_{#2}}

\def\numA{A}
\def\numG{G}

\def\mechA{\texttt{FreeMarket}}
\def\mechB{\texttt{SharedEndow}}
\def\mechC{\texttt{Propvincometax}}
\def\mechD{\texttt{SocialPlanner}}


\def\scenarioA{\textbf{Uniform}}
\def\scenarioB{\textbf{Privileged}}
\def\scenarioC{\textbf{Unequal-utility}}
\def\scenarioD{\textbf{Islands}}


\newcommand{\indep}[1]{\texttt{Indep}-$#1$}
\newcommand{\rewshare}[1]{\texttt{RewShare}-$#1$}


\def\SimName{\texttt{GatherBuild}}
\def\CleverName{EconRL}
\newcommand{\ourss}[1]{\CleverName{}-$#1$}
\newcommand{\ours}{\CleverName{{}}}


==> old.tex <==
\label{Protein and Language}
LMs are increasingly applied to large-scale protein sequence databases to learn embeddings for protein structure or function prediction recently~\citep{TomYoung2017RecentTI,KevinKYang2018LearnedPE,EhsaneddinAsgari2015ContinuousDR}. One important reason is that human languages and proteins share common characteristics. Such as the hierarchical organization~\citep{ferruz2022controllable, OFER20211750}, which means that the four different levels of protein structures (see Figure~\ref{fig_02}) analogy to letters, words, sentences, and texts of human languages to a certain degree. It illustrates that proteins and languages typically comprise modular elements that can be reused and rearranged. Moreover, the rules of protein folding, e.g., the hydrophilicity and hydrophobicity of amino acids, the principle of minimal frustration~\citep{bryngelson1995funnels} and the "folding funnel" landscapes of proteins~\citep{leopold1992protein}, etc., are similar to language grammars of linguistics. 
\begin{figure}[t]
	\centering
	\subfloat[Protein]
	{
		\label{fig_03_1}
		\includegraphics[width=0.62\linewidth]{figs/co_1.pdf}
	}
	\subfloat[Language]
	{
		\label{fig_03_2}
		\includegraphics[width=0.32\linewidth]{figs/co-2.pdf}
	}
	\caption{Comparisons of protein and language. (a) Relationship between a MSA and the residue contact of one protein in the alignment. The positions that coevolved are highlighted in red and light blue. Residues within these positions where changes occurred are shown in blue. Given such a MSA, one can infer correlations statistically found between two residues that these sequence positions are spatially adjacent, i.e., they are contacts~\citep{Zerihun2018BiomolecularSP, ochoa2014practical, vorberg2017bayesian}. (b) One grammatically complex sentence contains long-distance dependencies (shown in bold).}
	\label{fig_03}
\end{figure}

Figure~\ref{fig_03_1} shows a MSA and its statistical inference for residue contact of one protein. This illustrates that long-range dependencies exist between two residues; they may be far apart in the sequence but close in space resulting in coevolution. Similarly, long-distance dependencies, which pose a problem for machine translation and RNNs, also appeared in languages. Figure~\ref{fig_03_2} shows an example of language grammar rules that require agreement in the category of words that might be far from each other~\citep{choshen2019automatically}. All these similarities illustrate that researchers can deal with protein data using successful methods in NLP.

However, proteins are not human languages, despite these and other similarities. For example, the training of LMs often requires a massively large corpus, which needs tokenization, i.e., splitting the text into individual tokens or directly using words as tokens, which serves computational goals and, ideally, can also fulfil linguistic goals in NLP~\citep{EthanCAlley2019UnifiedRP, AliMadani2021DeepNL, KevinKYang2018LearnedPE, EhsaneddinAsgari2015ContinuousDR, DanOfer2021TheLO}. Compared with algorithms in NLP, protein tokenization methods still remain at a low level without a well-defined and biologically meaningful protein token algorithm~\citep{MaiHaVu2022AdvancingPL}. This may be a direction for unlocking the secrets of proteins.
\section{Language Models}
This section firstly introduces encoder architectures of LMs broadly falling into two categories: recurrent neural networks (RNNs) and attention mechanisms, especially for long short-term memory (LSTM)~\citep{GuillaumeLample2016NeuralAF} and transformers~\citep{vaswani2017attention}. Then we present the commonly-used pre-trained LMs and their developments.
\subsection{Recurrent Neural Networks (RNNs) and Long Short-term Memory (LSTM)}
The first example of LM was studied by Andrey Markov, who proposed the Markov chain in 1913~\citep{hayes2013first,li2022language}. After that, some machine learning methods, hidden Markov models (HMMs) and their variants particularly, are described and applied as fundamental tools in many fields, including biological sequences ~\citep{bishop1986maximum} where the goal is to recover a data sequence that is not immediately observable~\citep{chiu2020scaling, gales2008application,nicolai2013solving,domingos2015master,stigler2011complex,wong2013dna}.

Neural networks started to produce superior results in various NLP tasks since 2010s~\citep{ferruz2022controllable}. RNNs allow previous outputs to be used as inputs while having hidden states to exhibit temporal dynamic behaviours. Therefore, RNNs can use their internal states to process variable-length sequences of inputs that are useful and applicable in NLP tasks~\citep{agmls2009novel}. 
\begin{figure}[t]
	\centering
	\subfloat[RNNs]
	{
		\label{fig4-a}
		\includegraphics[width=0.52\linewidth]{figs/RNNs2.pdf}
	}
	\subfloat[LSTM cell]
	{
		\label{fig4-b}
		\includegraphics[width=0.42\linewidth]{figs/LSTM1.pdf}
	}
	\caption{Graphical explanation of RNNs and LSTM.}
	\label{fig_04}
\end{figure}

RNNs are typically shown in Figure~\ref{fig4-a}. In each timestep $t$, the input $x_{t}\in \mathbb{R}^l$, hidden $h_{t}\in \mathbb{R}^d$ and output state vectors $o_{t}\in \mathbb{R}^d$, where the superscripts $l$ and $d$ refer to the number of input features and the number of hidden units, respectively, are formulated as follows:
\begin{align*}
h_{t}&=g\left(W_{x}x_{t} + W_{h}h_{t-1} + b_h \right)\\
o_{t}&=g\left(W_{y}h_{t} + b_y \right)
\end{align*}
Where $W_x\in \mathbb{R}^{d\times l}$, $W_h\in \mathbb{R}^{d\times d}$ and $W_y\in \mathbb{R}^{d\times d}$ are the weights associated with the input, hidden and output vectors in the recurrent layer, and $b_h\in \mathbb{R}^{d}$, $b_y\in \mathbb{R}^{d}$ are the bias, which are shared temporally, $g$ is the activation function.

In order to deal with the vanishing gradient problem~\citep{hochreiter1991untersuchungen} that can be encountered when training traditional RNNs, LSTM networks were developed to process sequences of data. They presented superior capabilities in learning long-term dependencies~\citep{GuillaumeLample2016NeuralAF} with various applications such as time series prediction~\citep{schmidhuber2005evolino}, protein homology detection~\citep{hochreiter2007fast}, drug design~\citep{gupta2018generative}, etc. Unlike standard LSTM, bidirectional LSTM (BiLSTM) adds one more LSTM layer, reversing the information flow direction. This means it is capable of utilizing information from both sides and is also a powerful tool for modelling the sequential dependencies between words and phrases in a sequence~\citep{ma2021short}.

The LSTM architecture aims to provide a short-term memory that can last more timesteps, shown in Figure~\ref{fig4-b}, $\sigma$ and $\mathrm{tanh}$ represent the sigmoid and tanh layer. Forget gate layer in the LSTM is to decide what information is going to be thrown away from the cell state at timestep $t$, $x_{t}\in \mathbb{R}^l$, $h_t \in(-1,1)^d$ and $f_t \in(0,1)^d $ are the input, hidden state vectors and forget gate's activation vector. 
\begin{equation*}
f_t=\sigma(W_fx_t + U_fh_{t-1} +b_f )
\end{equation*}
Then, the input gate layer decides which values should be updated, and a tanh layer creates a vector of new candidate values, $\tilde{C}_t\in(-1,1)^d$ that could be added to the state, $i_t \in(0,1)^d$ is the input gate's activation vector.
\begin{align*}
i_t &=\sigma(W_ix_t + U_ih_{t-1} +b_i) \\
\tilde{C}_t &=\tanh (W_cx_t + U_ch_{t-1} +b_c)
\end{align*}
Next, we combine old state $C_{t-1}\in \mathbb{R}^d$ and new candidate values $\tilde{C}_t\in(-1,1)^d$ to create an update to the new state $C_t\in \mathbb{R}^d$.
\begin{equation*}
C_t=f_t \odot C_{t-1}+i_t \odot \tilde{C}_t
\end{equation*}
Finally, the output gate layer decides what parts of the cell state to be outputted, $o_t \in(0,1)^d$.
\begin{align*}
o_t &=\sigma (W_ox_t + U_oh_{t-1}+b_o) \\
h_t &=o_t \odot \tanh \left(C_t\right)
\end{align*}
where $\{W_f, W_i, W_c, W_o\} \in \mathbb{R}^{d \times l}, \{U_f, U_i, U_c, U_o\} \in \mathbb{R}^{d \times d}$ and $ \{b_f, b_i, b_c, b_o\} \in \mathbb{R}^d$ are weight matrices and bias vector parameters in the LSTM cell, $\odot$ means the pointwise multiplication.

\subsection{Attention Mechanism and Transformer}
Traditional Sequence-to-Sequence (Seq2Seq) models use RNNs or LSTMs as encoders and decoders~\citep{AlecRadford2017LearningTG} to process sequence and extract features for tasks. The final state of RNNs or LSTMs (better to say, encoders) must hold information for the entire input sequence, which may cause information loss. Therefore, traditional RNNs and LSTMs were soon superseded by attention mechanisms~\citep{DzmitryBahdanau2014NeuralMT, XuHan2021PreTrainedMP}, which help look at all hidden states from the encoder sequence for making predictions and were first applied for sequence modelling in machine translation~\citep{bahdanau2014neural}. 

The attention layer can access all previous states and learn their importance to weight them. Based solely on attention mechanisms, Google Brain released Transformer~\citep{vaswani2017attention} in 2017, a new network architecture dispensing with recurrence and convolutions entirely. This led to the development of pre-trained models, e.g., Bidirectional encoder representations from transformers (BERT)~\citep{JacobDevlin2022BERTPO} and Generative pre-trained transformer (GPT)~\citep{AlecRadford2022ImprovingLU,AlecRadford2022LanguageMA,TomBBrown2020LanguageMA}, which were trained with large language datasets. Unlike RNNs, Transformer processes the entire input all at once, using stacked self-attention layers for both the encoder and decoder. Each layer consists of a multi-head attention module followed by a feed-forward module with a residual connection and normalization. The vanilla single-head attention is called "Scaled Dot-Product Attention" and operates as follows:
\begin{equation*}
\operatorname{Att}(Q, K, V)=\operatorname{Softmax}\left(\frac{Q K^{\top}}{\sqrt{d}}\right) V
\end{equation*}
where $Q, K, V \in \mathbb{R}^{l \times d}$ are $d$-dimensional vector representations of $l$ words in sequences of queries, keys
and values, respectively. Multi-head attention allows the model to attend to information from different representation subspaces in parallel jointly. \begin{align*}
\operatorname{MultiHead}\left(Q, K, V\right)&=\mathrm{Concat}\left(\mathrm{head_1}, \ldots, \mathrm{head}_{\mathrm{h}}\right)W^O\\ 
\mathrm{where} \ \mathrm{head}_{\mathrm{i}}&=\mathrm{Att}\left(Q W_i^Q, K W_i^K, V W_i^V\right) 
\end{align*}
where the projections are parameter matrices $W_i^Q \in \mathbb{R}^{d \times d_i}, W_i^K \in \mathbb{R}^{d \times d_i}, W_i^V \in \mathbb{R}^{d \times d_i}$ and $W^O \in \mathbb{R}^{hd_i \times d}, d_i=d/h$, there are $h$ parallel attention layers or heads. Moreover, in Transformer, the position-wise feed-forward networks consist of two linear transformations with a ReLU activation in between, and positional encoding is added to the input embedding at the bottoms of the encoder and decoder stacks to make use of the order of the sequence.
\subsection{Pre-trained Language Models}
In order to train effective deep neural models focusing on storing knowledge for specific tasks with limited human-annotated data, transfer learning with a pre-training phrase and a fine-tuning stage has been adopted~\citep{XuHan2021PreTrainedMP,SebastianThrun1998LearningTL,SinnoJialinPan2010ASO}. In recent years, we have witnessed a rapid development of pre-trained LMs that have been widely used in NLP and computer vision, etc. Due to its prominent nature, the transformer gradually becomes a standard neural architecture for natural language understanding and generation. It also serves as the most commonly-used backbone neural architecture for pre-trained models as they have achieved state-of-the-art results on almost all NLP tasks. This indeed subverted our current perception of the performance of deep learning models, thus drawing more attention. An overview of some typical pre-trained LMs in general domains is shown in Table~\ref{Table_LMs}.
\begin{table*}[t]
	\caption{Representative pre-trained LMs in general domains}
	\label{Table_LMs}
	\setlength{\tabcolsep}{2.8pt}
	\centering
	\small
	\begin{adjustbox}{max width=\linewidth}
		\begin{threeparttable} %
			\begin{tabular}{lllll}
				\toprule 
				Model & Network & Objective &$\#$Params. &  Comments  \\
				\hline 
				ELMo~\citep{MatthewEPeters2018DeepCW}  &LSTM &Bidirectional LM & 93.6M & the first deep contextualized word representation\\
				GPT~\citep{AlecRadford2022ImprovingLU} &Transformer &Autoregressive LM & 110M & a pre-trained LM for predicting the next word\\
				BERT~\citep{JacobDevlin2022BERTPO}&Transformer& Masked LM &340M & the most commonly-used LM for predicting masked tokens\\
				Transformer-XL~\citep{ZihangDai2019TransformerXLAL} & Transformer  &Autoregressive LM & 257M & enabling learn dependencies beyond a fixed length \\
				XLM~\citep{GuillaumeLample2019CrosslingualLM} & Transformer& Multi-task &665M & cross-lingual pre-training \\
				Udify~\citep{DanKondratyuk201975L1} & BERT & Multi-task & $\sim$340M &leveraging a multilingual BERT self-attention model\\
				GPT-2~\citep{Radford2019} & Transformer& Autoregressive LM & 1.5B & larger model, more training data\\
				Grover~\citep{zellers2019grover}&GPT2 &Autoregressive LM & 1.5B 
				& defending against the general neural fake news\\
				XLNet~\citep{ZhilinYang2019XLNetGA} & BERT &Autoregressive LM & $\sim$340M & more training data, integrates ideas from Transformer-XL\\
				RoBERTa~\citep{YinhanLiu2019RoBERTaAR} & BERT & Masked LM & 355M & more training data, dynamic masking\\
				CTRL~\citep{NitishShirishKeskar2019CTRLAC} & Transformer &Autoregressive LM&1.63B& trained to control particular aspects of the generated text\\
				Megatron-LM~\citep{MohammadShoeybi2019MegatronLMTM} & Transformer & Autoregressive LM & 8.3B & a large transformer model\\
				ALBERT~\citep{ZhenzhongLan2019ALBERTAL} & BERT & Masked LM & 223M & a lite BERT\\
				DistillBERT~\citep{VictorSanh2019DistilBERTAD} & BERT & Masked LM & 65M & a distilled version of BERT\\
				SpanBERT~\citep{joshi2019spanbert} & BERT & Masked LM & $\sim$340M  & presenting and predicting the masked span \\
				MASS~\citep{KaitaoSong2019MASSMS} & Transformer & Seq2Seq LM & $\sim$307M & masked Seq2Seq pre-training\\
				MT-DNN~\citep{liu2019mt-dnn,liu2020mtmtdnn} & BERT & Multi-task & $\sim$340M &  for multiple natural language understanding tasks\\
				$\mathrm{MT-DNN}_{\mathrm{KD}}$~\citep{liu2019mt-dnn-kd} & MT-DNN & Multi-task & $\sim$340M & incorporating knowledge distillation \\
				ERNIE~\citep{ZhengyanZhang2019ERNIEEL} & BERT & Masked LM & $\sim$114M & incorporating knowledge graphs\\
				KnowBERT~\citep{MatthewEPeters2019KnowledgeEC} & BERT & Masked LM & $\sim$110M & incorporating knowledge bases into BERT \\
				KEPLER~\citep{XiaozhiWang2019KEPLERAU} & RoBERTa & Masked LM & $\sim$125M & incorporating knowledge embedding \\
				VideoBERT~\citep{ChenSun2019VideoBERTAJ} & BERT & Multimodal model & $\sim$340M & modelling between the visual and linguistic domain\\
				VisualBERT~\citep{LiunianHaroldLi2019VisualBERTAS} & BERT & Multimodal model & $\sim$110M & modelling a broad range of vision and language tasks\\
				ERNIE~\citep{YuSun2019ERNIEER} & BERT & Masked LM & $\sim$110M & a new masking strategy\\
				PEGASUS~\citep{zhang2020pegasus} & Transformer & Masked $\&$ Seq2Seq LM & 568M & for abstractive text summarization \\
				Unicoder-VL~\citep{GenLi2020UnicoderVLAU} & BERT & Multimodal model & $\sim$110M & cross-modal learning \\
				UNILM~\citep{unilmv2} & BERT & Bidirectional  $\&$ Seq2Seq LM & $\sim$110M & for natural language understanding and generation tasks\\
				Turing-NLG~\citep{JeffRasley2020DeepSpeedSO} & Transformer  &Autoregressive LM &17B& a hugely large LM\\
				ELECTRA~\citep{KevinClark2020ELECTRAPT} & BERT & Generator $\&$ Discriminator &335M &token detection\\
				GPT-3~\citep{TomBBrown2020LanguageMA} & GPT-2 & Autoregressive LM &175B & extending the model size\\
				T5~\citep{raffel2020exploring} & Transformer & Seq2Seq LM & 11B & producing new text as output\\
				Switch Transformer~\citep{WilliamFedus2021SwitchTS} & Transformer & Masked LM & 1.6T & increasing the pre-training speed \\
				BEIT~\citep{beit} & Transformer & Masked image model & 307M & a vision Transformer\\
				MT-NLG~\citep{ShadenSmith2022UsingDA} & Transformer & Autoregressive LM & 530B & the largest publicly monolithic transformer \\
				
				\toprule
			\end{tabular}
			\begin{tablenotes} %
				\item All examples report the largest model of their public series. Network displays high-level backbone models preferentially if they are used to initialize parameters. $\#$Param. means the number of parameters; M, millions; B, billions; T, trillions; $\&$ , and; $\sim$ means estimated data. Related terminologies are listed in Section~\ref{Notions and Terms}.
			\end{tablenotes} %
		\end{threeparttable}
	\end{adjustbox}
\end{table*}

\subsubsection{GPT and BERT}
With transformers as architectures and LM learning as objectives, BERT and GPT are the two landmarks that completely open the door towards the era of large-scale, deeply pre-trained LMs. 

GPT optimizes standard autoregressive language modelling during pre-training, which uses a transformer to model the conditional probability of each word and therefore, is powerful at predicting the next token in a sequence.
Formally, given an unsupervised corpus of tokens $\mathcal{X}=\left\{x_0, x_1, \ldots, x_n, x_n+1\right\}$, GPT applies a standard language modelling objective to maximize the following likelihood:
\begin{equation*}
\mathcal{L}(\mathcal{X})=\sum_{i=1}^{n+1} \log P\left(x_i \mid x_{i-k}, \ldots, x_{i-1} ; \Theta\right)
\end{equation*}
Where $k$ is the size of the context window, and the conditional probability $P$ is modelled using a network decoder with parameters $\Theta$. 

BERT uses a multi-layer bidirectional transformer encoder as its architecture. In the pre-training phase, BERT adopts the strategies of next-sentence prediction to understand sentence relationships with the help of a binary classifier and masked language modelling (MLM), which is powerful and applied in most self-supervised pre-training tasks. Formally, given a corpus consisting of tokens $\mathcal{X}=\left\{x_0, x_1, \ldots, x_n, x_n+1\right\}$, BERT maximizes the following likelihood: 
\begin{equation*}
\mathcal{L}(\mathcal{X})=\textstyle \sum_{x\in mask(\mathcal{X})} \log P ( x \mid \tilde{\mathcal{X}} ; \Theta)
\end{equation*}
where $mask(\mathcal{X})$ are the masked tokens, $\tilde{\mathcal{X}}$ is the result after masking some tokens in $\mathcal{X}$, and the probability $P$ is modeled by the transformer encoder with parameters $\Theta$.

\subsubsection{Post GPT and BERT Era}
After GPT and BERT, various of their improvements and variants have been proposed, as shown in Table~\ref{Table_LMs}. For example, researchers increased the size of models and datasets~\citep{YinhanLiu2019RoBERTaAR, ZhilinYang2019XLNetGA}, as large transformer models became the de facto standard in NLP on the basis of scaling laws, which can govern the dependence of overfitting on the model and dataset size for a given compute budget~\citep{JaredKaplan2020ScalingLF, JordanHoffmann2022TrainingCL}. The new masking strategies were proposed like entity-level masking, phrase-level masking~\citep{YuSun2019ERNIEER}, and span masking that masks the tokens consecutively according to the span length~\citep{joshi2019spanbert}, entity-level masking and phrase-level masking. Incorporating different data sources has also been developing as an important direction, such as utilizing multilingual corpora, and knowledge graphs~\citep{GuillaumeLample2019CrosslingualLM, MatthewEPeters2019KnowledgeEC}. Furthermore, because Pre-trained LMs are not data-hungry to labelled data and present better performance, they gradually stepped into different domains, including financial, computer vision and biomedical applications~\citep{araci2019finbert, BenyouWang2022PretrainedLM,YoshuaBengio2022ANP,TomasMikolov2013EfficientEO, lee2020biobert}, etc. 

\section{Protein Language Models}
As stated before, protein sequences corresponding to strings of amino-acid letters are a natural fit to most LMs, which are able to capture complex dependencies among these amino acids~\citep{OFER20211750}. pLMs have been developed and emerged as promising approaches for learning protein sequences. In this section, we first introduce LSTM pLMs, then present transformer pLMs with different implementation strategies and applications elaborately, especially the pLMs aimed at PSP. We listed a group of representative pLMs in Table~\ref{Table_pLMs}. The (pre-) training databases that appeared in this table are listed in Table~\ref{datasets}, where the CullPDB~\citep{GuoliWang2005PISCESRI} is a secondary structure prediction dataset.
\subsection{LSTM Protein Language Models}
\cite{MichaelSchantzKlausen2018NetSurfP20IP} trained a combination of convolutional and LSTM neural networks to predict protein structural features, solvent accessibility (SA), secondary structure (SS), structural disorder, and torsion angles ($\varphi$, $\psi$) for each residue of the input sequences. SPIDER3-Single~\citep{RhysHeffernan2018SinglesequencebasedPO} modelled on the single sequence instead of relying on evolutionary information from MSAs. Having similar training objectives and backbone architectures, such kind of examples are DeepPrime2Sec~\citep{EhsaneddinAsgari2019DeepPrime2SecDL}, SPOT-1D-Single~\citep{JaspreetSingh2021SPOT1DSingleIT}. Furthermore, DeepBLAST~\citep{JamesTMorton2020ProteinSA}, SPOT-1D-LM~\citep{JaspreetSingh2021SPOT1DLMRA} and SPOT-Contact-Single~\citep{JaspreetSingh2021SPOTContactSingleIS} are the usages of pre-trained pLMs to get embeddings for downstream tasks like contact map prediction, function prediction, etc.

However, \cite{RoshanRao2019EvaluatingPT} (TAPE) benchmarked a group of protein models across a panel of tasks, concluding that there exist opportunities for specific innovative design of protein models and training methods for vanilla LSTMs and Transformers. Methods specified for protein data processing have been researched and tested.

Without structural or evolutionary data, UniRep~\citep{EthanCAlley2019UnifiedRP} summarized arbitrary protein sequences into fixed-length vectors by multiplicative long-/short-term-memory (mLSTM)~\citep{BenKrause2016MultiplicativeLF}. Analogous to UniRep, UDSMProt~\citep{Strodthoff:2019universal} and SeqVec~\citep{MichaelHeinzinger2019ModelingTL} used LSTM or its variants to remember long-range dependencies for protein sequences to get rich representations that can be transferred and retrieved afterwards. ProSE~\citep{TristanBepler2021LearningTP} extra added structural supervision by residue-residue contact loss and structural similarity prediction loss to better capture the semantic organization of proteins and improved the ability to predict protein functions instead of using the masking loss only. Besides, \cite{TristanBepler2019LearningPS} proposed a soft symmetric alignment mechanism to measure similarities between sequence embeddings. CPCProt~\citep{AmyXLu2020SelfSupervisedCL} learned protein embeddings by formalizing the InfoNCE loss for the principle of mutual information maximization. All these models demonstrate the LSTM-like pLMs' ability to capture some biological properties of proteins.
\subsection{Transformer Protein Language Models}
\begin{figure}[t]
	\centering
	\subfloat[ESM-1b]
	{
		\label{ESM-1b}
		\includegraphics[width=0.95\linewidth]{figs/ESM-1b-1.pdf}
	}\\
	\subfloat[ESM-MSA]
	{
		\label{ESM-MSA}
		\includegraphics[width=0.95\linewidth]{figs/ESM-MSA-1.pdf}
	}
	\caption{Core modules of ESM-1b and ESM-MSA.}
	\label{ESM}
\end{figure}
\cite{AhmedElnaggar2021ProtTransTC} have trained six successful LMs (T5, ELECTRA, ALBERT, XLNet, BERT, and Transformer-XL, listed in Tabel~\ref{Table_LMs}) on protein sequences containing 393 billion amino acids using many resources (5616 GPUs and one TPU Pod). ESM-1b~\citep{AlexanderRives2019BiologicalSA} employed a deep Transformer (shown in Figure~\ref{ESM-1b}) and a masking strategy to build up complex representations that incorporate context from across the sequence. The results of ProtTrans~\citep{AhmedElnaggar2021ProtTransTC} and ESM-1b implied that large-scale pLMs have the advantage of learning the grammar of proteins even without using evolutionary information. Like approaches in NLP that change masking strategy, \cite{MatthewBAMcDermott2021AdversarialCP} updated the random masking scheme with a fully differentiable adversarial masking model. PMLM~\citep{LiangHe2022PretrainingCP} considered the dependency among masked tokens to capture the correlations (coevolution) of inter-residues, which was demonstrated to improve the performance on the TAPE contact benchmark. 
\subsubsection{Multi-source Knowledge Enhancement of Protein Representations}
Extra information, including MSAs, functions, structures and biological priors, may enrich protein embeddings. In detail, firstly, MSA Transformer~\citep{RoshanRao2021MSAT} extended the transformer LMs to deal with sets of sequences as input by alternating attention over rows and columns, shown in Figure~\ref{ESM-MSA}. Its internal representations enable high-quality unsupervised structure learning with an order of magnitude fewer parameters than contemporaneous pLMs. Secondly, ProteinBERT~\citep{DanOfer2021ProteinBERTAU} was pre-trained on protein sequences and Gene Ontology (GO) annotations which can be encoded as a binary vector. The learned embeddings contain information from both sequence and GO annotation to predict diverse protein functions~\citep{MAshburner2000GeneOT}; likewise, OntoProtein~\citep{NingyuZhang2022OntoProteinPP} considered GO as a factual knowledge graph, which was used to enhance protein representations. Finally, \cite{SanaaMansoor2021TowardMG} encoded two types of protein information (sequence and structure) through joint training in a semi-supervised manner. \cite{TristanBepler2021LearningTP} have carried out multi-task with structural supervision, leading to an even better-organized embedding space. STEPS~\citep{CanChen2022StructureawarePS} tried to correlate the embeddings learned from sequence and structure by pseudo bi-level optimization. 

However,~\cite{WeijieLiu2019KBERTEL} indicated that not all external knowledge is beneficial for downstream tasks. Thanks to the construction of benchmarks which can give relatively fair results of different methods. PEER benchmarks~\citep{MinghaoXu2022PEERAC} were built for protein sequence understanding, including protein function and structure prediction, protein-protein interaction prediction, protein-ligand interaction prediction tasks, etc. Its results showed that selecting suitable auxiliary tasks can boost different models' performance. Therefore, it is necessary to inject external features and design algorithms carefully and adequately.
\subsubsection{Transformer Models Designed for Protein Structure Prediction}
\begin{figure*}[h]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{figs/Evoformer.pdf}
	\end{center}
	\caption{Evoformer block.}
	\label{Evoformer}
\end{figure*}
Early pLMs tend to predict structural features~\citep{MichaelSchantzKlausen2018NetSurfP20IP, RhysHeffernan2018SinglesequencebasedPO, EhsaneddinAsgari2019DeepPrime2SecDL,JunwenLuo2020SelfSupervisedRL, JaspreetSingh2021SPOTContactSingleIS, RoshanRao2021TransformerPL, MagnusHaraldsonHie2022NetSurfP30AA, ShaunMKandathil2020DeepLP, MichaelHeinzinger2022ContrastiveLO}, like SS, SA, torsion angles, remote homology, and contact map, etc., which are useful for constructing protein 3D structures. Current pLMs tend to predict PSP end-to-end, which are introduced as follows. 

Evoformer is the core module (encoder) of the famous network, AF2~\citep{JohnMJumper2021HighlyAP}, which is repeated 48 times with no shared weights (shown in Figure~\ref{Evoformer}). It uses a variant of axial attention~\citep{JonathanHo2019AxialAI}, including row-wise gated self-attention with pair bias and column-wise gated self-attention, to process the MSA representation, which is transitioned by a 2-layer neural network, then used to update the pair representation by an outer product mean block, containing linear transforms, outer product, and mean, etc. In order to make the pair representation in the embedding space satisfy the demand of consistency, like the triangle inequality on distances, a triangle multiplicative update block and a triangle self-attention block were designed. The former updates the pair representation by combining information within each triangle of graph edges, while the latter operates self-attention around graph nodes. These ingenious designs let the output of Evoformer produce more insightful patterns for accurate PSP. Besides,~\cite{MingyangHu2022ExploringE} have shown that pLMs, especially those trained for PSP, like Evoformer, are valuable and general-purpose for various structure and function tasks. 

AminoBERT~\citep{RatulChowdhury2021SinglesequencePS} adopted a transformer to learn latent information from a single sequence, whose representation is inputted in a recurrent geometric network to generate the backbone structure of a protein. ESM-2~\citep{ZemingLin2022LanguageMO} is the largest pLM to date, extending ESM-1b and having parameters up to 15 billion, which has achieved the lowest validation perplexity and highest TM-score~\citep{YangZhang2005TMalignAP} on CASP14 compared with other smaller ESM models. The results indicated that improving the model sizes of pLMs is able to improve the PSP performance with little or no evolutionary information. OmegaPLM~\citep{RuidongWu2022HighresolutionDN} was trained with a stack of efficient GAU layers~\citep{WeizheHua2022TransformerQI} to get single- and pairwise-residue embeddings, which are expected to contain structural and functional information by different masking strategies, including random masking, sequential masking, and span masking~\citep{joshi2019spanbert}. In GAU, gate operation is applied after the attention aggregation and uses $\text{relu}^2(\cdot)$ to replace the conventional $\text{softmax}(\cdot)$, which performs better in terms of both computation speed and convergence rate in original experiments. AntiBERTy~\citep{JeffreyARuffolo2022FastAA} was pre-trained on antibody sequences to produce contextual embeddings for subsequent antibody structure prediction.

\subsubsection{Other Applications}
In terms of sequence generation, ProGen~\citep{madani2020progen} was trained on sequences conditioned on a set of protein properties like function or affiliation with a particular organism, and the training database contains about 280 million protein sequences and associated properties from different datasets. Compared with MSA Transformer~\citep{RoshanRao2021MSAT}, MSA2Prot~\citep{BeplerTristan2022FewSP} is a MSA-to-protein transformer, developed axial attention and cross attention for transformer encoder and decoder to model sequence probabilities autoregressively. Other methods include ProtGPT2~\citep{NoeliaFerruz2022ADU},  RITA~\citep{hesslow2022rita}, and ProGen2~\cite{ErikNijkamp2022ProGen2ET} (up to 6.4 billion parameters), etc.

Other than the models mentioned above, a group of pLMs are developed and trained for different purposes. For example, 
ESM-1v~\citep{meier2021language}, Tranception~\citep{PascalNotin2022TranceptionPF} enabled the prediction of the effects of mutations. Structured Transformer~\citep{JohnIngraham2019GenerativeMF}, ESM-IF1~\citep{hsu2022learning}, Fold2Seq~\citep{YueCao2021Fold2SeqAJ}, PeTriBERT~\citep{BaldwinDumortier2022PeTriBERTA}, ProteinMPNN~\citep{JDauparas2022RobustDL}, and~\citep{ZhangyangGao2022AlphaDesignAG, gao2022pifold, tan2022generative}, etc., were proposed for protein design, which is also referred to as the inverse protein folding problem, meaning recovering the native sequence of a protein from its tertiary structure (coordinates). ProtTucker~\citep{MichaelHeinzinger2022ContrastiveLO} utilized pLM and contrastive learning~\cite{chen2020simple,xia2022simgrace} strategy to improve the ability to recognize distant homologous, and other tasks, including profile prediction~\citep{PascalSturmfels2020ProfilePA}, evolutionary velocity prediction~\citep{BrianHie2021EvolutionaryVW}, enzymatic active sites identification~\citep{LocKwateDassi2021IdentificationOE}, etc. 

\begin{table*}[t]
	\caption{List of representative pLMs}
	\label{Table_pLMs}
	\setlength{\tabcolsep}{2.8pt}
	\centering
	\small
	\begin{adjustbox}{max width=\linewidth}
		\begin{threeparttable} %
			\begin{tabular}{llllllll}
				\toprule 
				Model and Repository&Approach & Input & Network &$\#$Embedding &$\#$Param.  & Pre-training Database \\
				\hline 
				\href{https://services.healthtech.dtu.dk/service.php?NetSurfP-2.0}{NetSurfP-2.0}~\citep{MichaelSchantzKlausen2018NetSurfP20IP} & Supervised & MSA, Structure & CNN, BiLSTM & 2048 & N/A & PDB, UniRef30 \\
				
				\href{http://sparks-lab.org}{SPIDER3-Single}~\citep{RhysHeffernan2018SinglesequencebasedPO} & Supervised & Sequence, Structure & LSTM-BRNN~\citep{RhysHeffernan2017CapturingNI} & 1024, 512 & N/A & 12442 proteins \\
				\href{https://github.com/Rostlab/SeqVec}{SeqVec}~\citep{MichaelHeinzinger2019ModelingTL}&Unsupervised  &Sequence & ELMo & 1024 &$\sim$93.6M & UniRef50\\
				
				\href{https://github.com/churchlab/Unirep}{UniRep}~\citep{EthanCAlley2019UnifiedRP}&Unsupervised & Sequence & mLSTM~\citep{BenKrause2016MultiplicativeLF} & 1900 &$\sim$18.2M & UniRef50\\
				
				\href{https://github.com/tbepler/protein-sequence-embedding-iclr2019}{SSA}~\citep{TristanBepler2019LearningPS}& Supervised & Sequence, Structure & BiLSTM & 100, 512 & N/A & Pfam, SCOP\\
				
				\href{https://github.com/ehsanasgari/DeepPrime2Sec}{DeepPrime2Sec}~\citep{EhsaneddinAsgari2019DeepPrime2SecDL} & Supervised & MSA, Sturcture & ELMo, CNN, BiLSTM & N/A &  N/A & UniRef50, Swiss-Prot, CullPDB \\
				
				\cite{JohnIngraham2019GenerativeMF} & Unsupervised & Structure & Transformer & 128 & N/A & CATH4.2 \\
				
				\multirow{2}{*}{\href{https://github.com/songlab-cal/tape}{TAPE}~\citep{RoshanRao2019EvaluatingPT}} & \multirow{2}{*}{Unsupervised} & \multirow{2}{*}{Sequence} & LSTM& 2048 & N/A & \multirow{2}{*}{Pfam} \\
				&&&Transformer & 768& 38M & \\
				\href{https://github.com/facebookresearch/esm}{ESM-1b}~\citep{AlexanderRives2019BiologicalSA} & Unsupervised & Sequence & Transformer & 1280& 650M & UniParc\\
				
				\href{https://github.com/nstrodt/UDSMProt}{UDSMProt}~\citep{Strodthoff:2019universal} & Unsupervised & Sequence & LSTM & 400 & $\sim$24M & Swiss-Prot\\
				
				\href{https://github.com/amyxlu/CPCProt}{$\mathrm{CPCProt}_{\mathrm{GRU \_ large}}$}~\citep{AmyXLu2020SelfSupervisedCL} & Unsupervised & Sequence & GRU~\citep{cho2014properties} & 1024 & 8.4M & Pfam \\
				\href{https://github.com/amyxlu/CPCProt}{$\mathrm{CPCProt}_{\mathrm{LSTM}}$}~\citep{AmyXLu2020SelfSupervisedCL} & Unsupervised & Sequence & LSTM & 2048 & 71M & Pfam \\
				
				\cite{PascalSturmfels2020ProfilePA} & Supervised & MSA & Transformer & N/A & N/A & Pfam \\
				
				\href{https://github.com/lucidrains/progen}{ProGen}~\citep{madani2020progen} & Unsupervised & Sequence, Property & Transformer & 1028 & 1.2B & $\sim$280M proteins\\
				
				
				\href{https://github.com/agemagician/ProtTrans}{ProtTXL}~\citep{AhmedElnaggar2021ProtTransTC} & Unsupervised & Sequence & Transformer-XL & 1024 & 562M & BFD100, UniRef100 \\
				\href{https://github.com/agemagician/ProtTrans}{ProtBert}~\citep{AhmedElnaggar2021ProtTransTC} & Unsupervised & Sequence & BERT & 1024 & 420M & BFD100, UniRef100 \\
				\href{https://github.com/agemagician/ProtTrans}{ProtXLNet}~\citep{AhmedElnaggar2021ProtTransTC} & Unsupervised & Sequence & XLNet & 1024 & 409M &UniRef100\\
				\href{https://github.com/agemagician/ProtTrans}{ProtAlbert}~\citep{AhmedElnaggar2021ProtTransTC} & Unsupervised & Sequence & ALBERT & 4096 & 224M &UniRef100\\
				\href{https://github.com/agemagician/ProtTrans}{ProtElectra}~\citep{AhmedElnaggar2021ProtTransTC} & Unsupervised & Sequence & ELECTRA & 1024 & 420M &UniRef100\\
				\href{https://github.com/agemagician/ProtTrans}{ProtT5}~\citep{AhmedElnaggar2021ProtTransTC} & Unsupervised & Sequence & T5 & 1024 & 11B &UniRef50, BFD100\\
				
				\href{https://github.com/jas-preet/SPOT-1D-Single}{SPOT-1D-Single}~\citep{JaspreetSingh2021SPOT1DSingleIT} & Supervised & Sequence, Structure & BiLSTM, ResNet~\citep{KaimingHe2016IdentityMI} & 256 & N/A & 39120 proteins \\
				
				\href{https://github.com/tbepler/prose}{ProSE}~\citep{TristanBepler2021LearningTP} &Supervised & Sequence, Structure & BiLSTM & 1024 & 1M & UniRef90, SCOPe \\
				
				\href{https://github.com/facebookresearch/esm}{MSA Transformer}~\citep{RoshanRao2021MSAT} & Unsupervised & MSA & Transformer & 768 & 100M & UniRef50, UniClust30\\
				\href{https://github.com/facebookresearch/esm}{ESM-1v}~\citep{meier2021language} & Unsupervised & Sequence & ESM-1b & 1280 & 650M & UniRef90\\
				\href{https://github.com/facebookresearch/esm}{ESM-IF1}~\citep{hsu2022learning} & Supervised & Sequence, Structure &GVP~\citep{BowenJing2020LearningFP}, Transformer & 512 & 142M & UniRef50, CATH\\
				\multirow{2}{*}{\href{https://github.com/nadavbra/protein_bert}{ProteinBERT}~\citep{DanOfer2021ProteinBERTAU}} & \multirow{2}{*}{Supervised} & Sequence &  \multirow{2}{*}{Transformer} & \multirow{2}{*}{128, 512} & \multirow{2}{*}{$\sim$16M} & \multirow{2}{*}{UniRef90} \\
				& & GO annotation & & & &\\
				
				\href{https://github.com/IBM/fold2seq}{Fold2Seq}~\citep{YueCao2021Fold2SeqAJ} & Supervised & Sequence, Structure & Transformer & 256 & N/A & CATH4.2 \\
				
				\href{https://github.com/aqlaboratory/rgn2}{AminoBERT}~\citep{RatulChowdhury2021SinglesequencePS} & Unsupervised & Sequence & Transformer & 3072 & N/A & UniParc \\
				\href{https://github.com/deepmind/alphafold}{Evoformer}~\citep{JohnMJumper2021HighlyAP} & Supervised & MSA, Structure & Attention network &  384, 128 & 93M & PDB, BFD, UniClust30, etc.\\
				\href{https://github.com/HeliXonProtein/OmegaFold}{OmegaPLM}~\citep{RuidongWu2022HighresolutionDN}& Unsupervised & Sequence & GAU~\citep{WeizheHua2022TransformerQI} & 1280 & 670M & UniRef50 \\
				\href{https://github.com/zjunlp/OntoProtein}{OntoProtein}~\citep{NingyuZhang2022OntoProteinPP} & Supervised & Sequence, GO & ProtBert, BERT & 1024 & N/A & ProteinKG25 \\
				PeTriBERT~\citep{BaldwinDumortier2022PeTriBERTA} & Unsupervised & Sequence, Structure & BERT & 3072 & <40M & AlphaFoldDB \\
				MSA2Prot~\citep{BeplerTristan2022FewSP} & Unsupervised & MSA & Transformer & 768 & N/A & Pfam \\
				
				PMLM~\citep{LiangHe2022PretrainingCP} & Unsupervised & Sequence & Transformer & 1280 & 715M & UniRef50 \\
				
				\href{https://github.com/salesforce/progen}{ProGen2}~\citep{ErikNijkamp2022ProGen2ET} & Unsupervised & Sequence & Transformer & 4096 & 6.4B & UniRef90, BFD30\\
				\href{https://github.com/OATML-Markslab/Tranception}{Tranception}~\citep{PascalNotin2022TranceptionPF} & Unsupervised & Sequence & Transformer & 1280 & 700M & UniRef100 \\
				
				\href{https://huggingface.co/nferruz/ProtGPT2}{ProtGPT2}~\citep{NoeliaFerruz2022ADU} & Unsupervised & Sequence & GPT-2 & 1280 & 738M&  UniRef50 \\
				\href{https://github.com/lightonai/RITA}{RITA}~\citep{hesslow2022rita} & Unsupervised & Sequence & GPT-3 & 2048 & 1.2B & UniRef100 \\
				\href{https://github.com/facebookresearch/esm}{ESM-2}~\citep{ZemingLin2022LanguageMO} & Unsupervised & Sequence & Transformer & 5120 & 15B & UniRef50 \\
				
				
				
				\toprule
			\end{tabular}
			\begin{tablenotes} %
				\item All examples report the largest model of their public series, the model name with colour is linked with GitHub or server page. Approach and database are listed for the pre-training stage, and the latter is elaborated on in Section~\ref{Databases}. Input is classified into protein sequence, MSA, structure (structural features or coordinates), and function. Network displays high-level backbone models preferentially if they are used. $\#$Embedding means the dimension of embeddings; $\#$Param., the number of parameters of network; M, millions; B, billions; T, trillions; N/A, null; $\&$, and; $<$, less than; $\sim$ estimated data. 
			\end{tablenotes} %
		\end{threeparttable}
	\end{adjustbox}
\end{table*}

\section{Methods of Protein Structure Prediction (PSP)}
This section mainly introduces different methods that work for different levels of prediction of protein structures, including traditional methods and deep learning methods. Among them, pLM-based models function importantly and significantly influence protein tasks.

\tikzstyle{leaf}=[draw=hiddendraw,
rounded corners,minimum height=1.2em,
fill=hidden-orange!40,text opacity=1, align=center,
fill opacity=.5,  text=black,align=left,font=\scriptsize,
inner xsep=3pt,
inner ysep=1pt,
]
\begin{figure*}[t]
	\centering
	\begin{forest}
		for tree={
			forked edges,
			grow=east,
			reversed=true,
			anchor=base west,
			parent anchor=east,
			child anchor=west,
			base=middle,
			font=\footnotesize,
			rectangle,
			draw=hiddendraw,
			rounded corners,align=left,
			minimum width=2.5em,
			minimum height=1.2em,
			s sep=6pt,
			inner xsep=3pt,
			inner ysep=1pt,
		},
		where level=1{text width=4.5em}{},
		where level=2{text width=6em,font=\scriptsize}{},
		where level=3{font=\scriptsize}{},
		where level=4{font=\scriptsize}{},
		where level=5{font=\scriptsize}{},
		[Structural\\Features, edge=hiddendraw
		[1D\\Features,text width=3em, edge=hiddendraw
		[ANN, text width=3.8em, edge=hiddendraw
		[
		\cite{LHHolley1989ProteinSS}{,}
		\cite{BurkhardRost1993ImprovedPO}{,}
		DBNN~\citep{XinQiuYao2008ADB}{,}\\
		DNSS~\citep{MatthewSpencer2015ADL}{,}
		\cite{HarisHasic2017AHM}{,}
		\href{http://sparks-lab.org/}{SPIDER2}~\citep{RhysHeffernan2015ImprovingPO}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[CNN, text width=3.8em, edge=hiddendraw
		[
		\cite{AkosuaBusia2016ProteinSS}{,}
		MUST-CNN~\citep{ZemingLin2016MUSTCNNAM}{,}\\
		\href{http://raptorx2.uchicago.edu/StructurePropertyPred/predict/}{RaptorX-Property}~\citep{ShengWang2016RaptorXPropertyAW}{,}
		GSN~\citep{JianZhou2014DeepSA}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[RNN, text width=3.8em, edge=hiddendraw
		[\href{http://scratch.proteomics.ics.uci.edu/}{SSpro/ACCpro5}~\citep{ChristopheMagnan2014SSproACCpro5A}{,}
		\href{http://sparkslab.org}{SPIDER3}~\citep{RhysHeffernan2017CapturingNI}{,}\\
		\cite{SrenKaaeSnderby2014ProteinSS}{,}
		\href{http://sparks-lab.org}{SPIDER3-Single}~\citep{RhysHeffernan2018SinglesequencebasedPO}{,}\\
		\href{http://distilldeep.ucd.ie/porter/}{Porter 5}~\citep{MirkoTorrisi2018Porter5S}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[Hybrid, text width=3.8em, edge=hiddendraw
		[
		\href{https://services.healthtech.dtu.dk/service.php?NetSurfP-2.0}{NetSurfP-2.0}~\citep{MichaelSchantzKlausen2018NetSurfP20IP}{,}
		\href{https://github.com/ehsanasgari/DeepPrime2Sec}{DeepPrime2Sec}~\citep{EhsaneddinAsgari2019DeepPrime2SecDL}{,}\\
		MASSP~\citep{BianLi2020AMD}{,}
		\href{https://sparks-lab.org/server/spot-1d-single/}{SPOT-1D-Single}~\citep{JaspreetSingh2021SPOT1DSingleIT}{,}
		\href{http://qianglab.scst.suda.edu.cn/crrnn2/}{CRRNN2}~\citep{BuzhongZhang2021MultitaskDL}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[Transformer, text width=3.8em, edge=hiddendraw
		[
		SPOT-1D-LM~\citep{JaspreetSingh2021SPOT1DLMRA}{,}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		]
		[2D\\Features,text width=3em, edge=hiddendraw
		[ANN, text width=3.8em, edge=hiddendraw
		[
		\href{https://predictioncenter.org/}{MetaPSICOV2}~\citep{DanielWABuchan2018ImprovedPC}{,}
		DeepCDpred~\citep{ShuangxiJi2018DeepCDpredID}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[CNN, text width=3.8em, edge=hiddendraw
		[
		RaptorX-Contact~\citep{ShengWang2016AccurateDN}{,}
		\href{https://github.com/multicom-toolbox/DNCON2/}{DNCON2}~\citep{BadriAdhikari2017DNCON2IP}{,}\\
		\href{https://github.com/largelymfs/deepcontact}{DeepContact}~\citep{YangLiu2017EnhancingEC}{,}
		\href{https://github.com/psipred/DeepCov}{DeepCov}~\citep{DavidTJones2018HighPI}{,}
		\cite{JinLi2021StudyOR}{,}\\
		\href{https://github.com/multicom-toolbox/deepdist}{DeepDist}~\citep{TianqiWu2020DeepDistRI}{,}
		\href{https://github.com/ba-lab/pdnet/}{PDNET}~\citep{BadriAdhikari2020AFO}{,}
		\href{https://github.com/multicom-toolbox/deepdist}{REALDIST}~\citep{BadriAdhikari2020REALDISTRP}{,}\\
		\href{https://seq2fun.dcmb.med.umich.edu//TripletRes/}{TripletRes}~\citep{YangLi2020DeducingHP}{,}
		\href{https://github.com/ElofssonLab/PconsC4}{PconsC4}~\citep{MircoMichel2019PconsC4FA}{,}
		\href{http://huanglab.phys.hust.edu.cn/DeepHomo/}{DeepHomo}~\citep{YumengYan2021AccuratePO}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[Hybrid, text width=3.8em, edge=hiddendraw
		[
		\href{http://sparks-lab.org/jack/server/SPOT-Contact/}{SPOT-Contact}~\citep{JackHanson2018AccuratePO}{,}
		\cite{ChenChen2020CombinationOD}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[Transformer, text width=3.8em, edge=hiddendraw
		[\href{https://github.com/ jas-preet/SPOT-Contact-Single}{SPOT-Contact-Single}~\citep{JaspreetSingh2021SPOTContactSingleIS}{,}
		\cite{NicholasBhattacharya2021SingleLO}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		]	
		[Both,text width=3em, edge=hiddendraw
		[CNN, text width=3.8em, edge=hiddendraw
		[
		\href{https://github.com/psipred/DMPfold}{DMPfold}~\citep{JoeGGreener2018DeepLE}{,}
		\href{https://github.com/ShenLab/ThreaderAI}{ThreaderAI}~\citep{HaicangZhang2020TemplatebasedPO}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		[Hybrid, text width=3.8em, edge=hiddendraw
		[
		DMPfold2~\citep{ShaunMKandathil2020DeepLP}
		,leaf,text width=25.4em, edge=hiddendraw]
		]
		]	
		]
	\end{forest}
	\caption{Taxonomy of structural feature prediction methods. ANN, Artificial Neural Network; Hybrid means models use CNN- and RNN-based methods simultaneously. The model name with colour is linked with the official GitHub or server page.}
	\label{taxonomy_of_structural_methods}
\end{figure*}

\subsection{Structural Features Prediction}
Structural features include 1D features (SS, SA, torsion angles, contact density, etc.) and 2D features (contact map and distance map)~\citep{MirkoTorrisi2020DeepLM}, which are useful for predicting protein structures. In the early stages of PSP, instead of predicting atom coordinates directly, researchers tried to predict structural features to evaluate their methods and aid the process of PSP. Methods of structural feature prediction are classified in Figure~\ref{taxonomy_of_structural_methods}. 

In the late 1980s, \cite{LHHolley1989ProteinSS} have already worked for protein secondary structure prediction (SSP) based on a neural network. DBNN~\citep{XinQiuYao2008ADB} combined dynamic Bayesian networks and neural networks to achieve improvements in SSP. DeepCNF~\citep{ShengWang2015ProteinSS} integrated conditional random fields (CRF) and shallow convolutional neural networks to predict SS of 3-state (H, E, C) and 8-state (G, H, I, E, B, T, S, L). \cite{RhysHeffernan2017CapturingNI} employed LSTM and bidirectional recurrent neural networks (BRNNs), which are capable of capturing long-range interactions. MASSP~\citep{BianLi2020AMD} used multi-tiered neural networks, which are composed of a CNN and a LSTM neural network, to get 1D structural attributes. As for 2D structural features prediction, RaptorX-Contact~\citep{ShengWang2016AccurateDN} integrated sequence and evolutionary coupling information by two deep residual neural networks to predict contact maps.~\cite{ChenChen2020CombinationOD} presented an attention-based convolutional neural network for protein contacts, including a sequence attention module and a regional attention network. \cite{JinLi2021StudyOR} studied the inter-atom distance and inter-residue orientation by a ResNet network and then built 3D structure models constrained by the predicted mean and deviation through PyRoseatta~\citep{SidharthaChaudhury2010PyRosettaAS}. Similarly, DeepDist~\citep{TianqiWu2020DeepDistRI}, PDNET~\citep{BadriAdhikari2020AFO}, REALDIST~\citep{BadriAdhikari2020REALDISTRP}, etc., were also proposed to learn the real‑value inter‑residue distance by designing regression models, which is more difficult than multi-class classification problem~\citep{JinboXu2018DistancebasedPF} but stepping forward for PSP.

However, the structural feature prediction tasks do not generally have significant practical values since there is already highly accurate 3D structure data from AF2. Is it a thing of the past? Considering it from another perspective, it can still provide a reference for the results of various proposed methods and work for finding the relationships between protein sequence, structure, and function by mining more protein grammars. For example, \cite{NicholasBhattacharya2021SingleLO} have introduced a simplified attention layer, factored attention, to find the role of attention, which achieved nearly identical performance to the Potts model with far fewer parameters. Particularly, DeepHomo~\citep{YumengYan2021AccuratePO} aimed to predict inter-protein residue-residue contacts across homo-oligomeric protein interfaces by integrating multi-source information to remove the potential intra-protein contact noises that exist in the MSA. Geoformer~\citep{RuidongWu2022HighresolutionDN} refined the details of contact prediction to illustrate its effectiveness in resolving the problem of triangular inconsistency.

\subsection{Traditional Methods for PSP}
\cite{KimTSimons1997AssemblyOP} generated native-like structures from fragments of unrelated protein structures using Bayesian scoring functions and a simulated annealing procedure in the 1990s. TOUCHSTONE II~\citep{YangZhang2003TOUCHSTONEIA} proposed a parallel hyperbolic sampling algorithm used in the Monte Carlo simulation processes to accelerate the conformational search faster. \cite{CarolARohl2004ProteinSP} utilized the Rosetta algorithm for \emph{de novo} PSP, which can assemble fragments by a Monte Carlo strategy. Such a strategy was also adopted in QUARK~\citep{DongXu2012AbIP}. \cite{AndreaCavalli2007ProteinSD} used chemical shifts as structural restraints to help determine the conformations of proteins. Based on backbone chemical shifts, \cite{ChristopheSchmitz2012ProteinSD} stepped further on the quest for reliable PSP using pseudocontact shifts. EdaFold~\citep{DavidSimoncini2012APF} is a fragment-based PSP method via estimation of distribution algorithm that is learned from previously generated decoys. Stepping on this, a cluster-based model and an energy-based variation were provided by \cite{DavidSimoncini2017BalancingEA}. UniCon3D~\citep{DebswapnaBhattacharya2016UniCon3DDN} is a generative, probabilistic model using united-residue conformational search, sampling lower energy conformations with higher accuracy than traditional random sampling. 

Structural features like SS and contact maps appear to help the PSP. DCAFold~\citep{JoannaISulkowska2012GenomicsaidedSP} integrated contacts estimated from direct coupling analysis with an accurate knowledge of local information to fold proteins. FragFold ~\citep{TomaszKosciolek2014DeNS} used fragment assembly with both statistical potentials and predicted contacts. RASREC~\citep{TatjanaBraun2015CombiningEI} integrated evolutionary information in the form of intra-protein residue-residue contacts. CONFOLD~\citep{BadriAdhikari2015CONFOLDRC} developed a distance geometry algorithm using structural features as restraints. \cite{SergeyOvchinnikov2016ImprovedDN} used structural information during Rosetta conformational sampling and refinement to improve the model's accuracy. Besides, RBO Aleph~\citep{MahmoudMabrouk2015RBOAL} leveraged evolutionary and physicochemical information to predict contacts, used in conformational space search,
afterwards, similar instances are SCDE~\citep{GuiJunZhang2020SecondarySA}, TDFO~\citep{GuiJunZhang2020TwoStageDF}. 

\subsection{Deep Learning Methods for PSP: Past, Present, and Future}
\subsubsection{Structural Features-Based Methods}
DESTINI~\citep{MuGao2019DESTINIAD} has two main components: a fully convolutional residual neural network for contact prediction with a template-based structural modelling procedure. Other than the distance map between $C_\beta$ atoms, \cite{JianyiYang2019ImprovedPS} and \cite{JinLi2021StudyOR} predicted orientations between residues via residual networks, which theoretically fully define the relative positions of the backbone atoms of two residues. The protein 3D structure is obtained from these inter-residue geometrics by energy minimization, then refined by full-atom relaxation; the pipeline is shown in Figure~\ref{Rosetta}. AlphaFold~\citep{AndrewWSenior2020ImprovedPS} optimized the potential and constructed predicted distances between pairs of residues through a simple gradient descent algorithm, which can generate structures directly, ignoring exhausting sampling procedures. Structural features-based PSP models commonly have two steps: contact predicting and structure modelling, which have so far been restricted to the accuracy of individual components, even though scientists seek to utilize different information (MSAs, templates, biochemical properties, etc.). In contrast, end-to-end differentiable models have obtained remarkable achievements~\citep{YannLeCun2015DeepL}.
\begin{figure*}[h]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{figs/rosetta.pdf}
	\end{center}
	\caption{A pipeline of predicting structural features and protein 3D structure. (a) Inter-residue geometrics, including distances ($d$) and orientations, three dihedral ($\omega, \theta_{ij}, \theta_{ij}$) and two planar ($\phi_{ij}, \phi_{ji}$) angles. (b) Outline of the PSP based on structural features from MSA via energy minimization and full-atom relaxation.}
	\label{Rosetta}
\end{figure*}
\subsubsection{End-to-end PSP}
RGN~\citep{MohammedAlQuraishi2018EndtoEndDL} predicted torsional angles from protein sequences fed into computational units based on LSTM, which are sequentially translated into Cartesian coordinates to generate the predicted structure. \cite{AlbertCosta2021DistillationOM} harvested individual and contextual residual embeddings produced by MSA Transformer, assigned to nodes and edges to Graph Transformer~\citep{YunshengShi2020MaskedLP}. The birth of the highly-accurate model, AlphaFold2 (AF2)~\citep{JohnMJumper2021HighlyAP} has stimulated the development of end-to-end models for PSP.

AF2 can produce even near-experimental results in most cases, whose accuracy was vastly higher than that of other competing methods in CASP14. The overall model architecture of AF2 is exhibited in Figure~\ref{AF2}. In addition to the above-mentioned Evoformer as mentioned earlier (listed in Table~\ref{Table_pLMs}, shown in Figure~\ref{Evoformer}), AF2 also has a decoder, the structure module that has eight layers with shared weights with the pair and first row MSA representations from the Evoformer as input. Each layer updates the single representation and the backbone frames, parameterized as Euclidean transforms. The structure module mainly includes the Invariant Point Attention (IPA) module, which is a form of attention that acts on a set of frames and is invariant under global Euclidean transformations because of the invariant operation, L2-norm of the global transformed vector. Moreover, AF2 executes the network three times with minor extra training time, embedding the previous outputs as additional inputs, making the network more profound and relatively important. There are various models with incremental improvements on different aspects concerning AF2, reducing training time for FastFold~\citep{ShengganCheng2022FastFoldRA} and Uni-Fold~\citep{ZiyaoLi2022UniFoldAO}, faster MSA generation for ColabFold~\citep{mirdita2022colabfold}, denoising the searched MSA or generating virtual MSA for EvoGen~\citep{JunZhang2022FewShotLO} that is useful for proteins lacking sequence homology, and re-implementation of AF2(HelixFold~\citep{GuoxiaWang2022HelixFoldAE}, MEGA-Fold~\citep{SiruiLiu2022PSPMP}, OpenFold~\citep{Ahdritz_OpenFold_2021}).
\begin{figure}[t]
	\centering
	\subfloat[AF2]
	{
		\label{AF2}
		\includegraphics[width=0.95\linewidth]{figs/AF2.pdf}
	}\\
	\subfloat[RosettaFold]
	{
		\label{RosettaFold}
		\includegraphics[width=0.95\linewidth]{figs/rosettafold.pdf}
	}
	\caption{A simplified schematic of AF2 and RosettaFold architectures.}
	\label{AF2 and RosettaFold}
\end{figure}

As for another famous PSP work, RoseTTAFold~\citep{MinkyungBaek2021AccuratePO} (as shown in Figure~\ref{RosettaFold}), it is a three-track model with attention layers in which information flows back and forth at the 1D, 2D, and 3D levels between sequences, distances, and coordinates, which is mainly consisted of seven modules. Firstly, the MSA features are processed by attention over rows and columns, and then the processed features are aggregated by the outer product that can obtain the correlation (coevolution) between two residues in each sequence to update pair features, which are refined via axial attention. Next, the MSA features are also updated based on attention maps derived from pair features, which had a good agreement with the true contact map. Using these learned MSA and pair features as the node and edge embeddings and building a fully-connected graph, Graph Transformer is employed to estimate the initial 3D structure, and new attention maps can be derived from the current structure to update MSA features. Finally, 3D coordinates are refined by SE(3)-Transformer~\citep{FabianBFuchs2020SE3Transformers3R} based on updated MSA and pair features.

Because of the remarkable success of AF2 and RosettaFold, a set of research has emerged, e.g., the protein-peptide binders identification~\citep{LiweiChang2022AlphaFoldET}, applying to small molecules~\citep{MaartenLHekkelman2021AlphaFillET}, antibody structure prediction~\citep{JeffreyARuffolo2022FastAA}, protein complex structure prediction~\citep{RichardEvans2021ProteinCP, PatrickBryant2021ImprovedPO}, RNA 3D structure prediction~\citep{TaoShen2022E2Efold3DED}, and generating multiple protein conformations~\citep{RichardAStein2022SPEACH}, so on and so forth, which are introduced in the following two subsections. A set of representative methods for PSP and related tasks are shown in Table~\ref{Table_PSP}.

\subsubsection{Single Sequence Structure Prediction via pLMs}
\begin{figure*}[h]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{figs/OmegaFold.pdf}
	\end{center}
	\caption{Model architecture of OmegaFold.}
	\label{OmegaFold}
\end{figure*}
These mainstream PSP pipelines heavily rely on MSAs, which becomes a kind of bottleneck for the reason that it is time-consuming and resource-intensive to search for MSAs and templates. Besides, a protein sequence can theoretically determine its structure; MSA-aware models may memorize the determined structures of similar proteins for PSP, making it difficult for us to understand the mechanism of folding in reality. In order to predict structure from only sequences without MSAs, a set of recent works deemed pLMs can capture grammatically structural information from protein sequence databases. OmegaFold~\citep{RuidongWu2022HighresolutionDN} utilized OmegaPLM to obtain the residue and pairwise embeddings from a single sequence, which are fed into Geoformer. Different from the triangle multiplicative and triangle attention modules applied in Evoformer to enforce the edge representation to satisfy the triangle inequality of distances, Geoformer considers maintaining geometric consistency in the high-dimensional space as well as in the Euclidean space with the help of the structure module implemented by AF2. The model architecture is demonstrated in Figure~\ref{OmegaFold}. The results of contact predictions illustrated that accuracy improves while inconsistency drops with stacked Geoformer layers. Thus, OmegaFold enables accurate predictions on orphan proteins, similar to AF2 structures. Other than OmegaFold, a contemporaneous work, ESMFold~\citep{ZemingLin2022LanguageMO}, has trained large-scale pLMs (ESM2) to learn more structural and functional properties to replace the role of MSAs; similar examples are HelixFold-Single~\citep{XiaominFang2022HelixFoldSingleMP}, RGN2~\citep{RatulChowdhury2021SinglesequencePS}. While trRosettaX-Single~\citep{WenkaiWang2022SinglesequencePS} used pre-trained pLMs (ESM-1b) and retrained it based on supervised learning (s-ESM-1b), distilling knowledge from a pre-trained MSA-based network ($\text{Res2Net\_MSA}$) to the student network ($\text{Res2Net\_Single}$) to predict distance and orientations.
\subsubsection{Diversified Progress in the Protein Field}
\cite{JamesPRoney2022StateoftheArtEO} found that AlphaFold has the ability to learn a highly accurate biophysical energy function and find a low-energy conformation using co-evolutionary information, which is important for single-sequence PSP using physical principles~\citep{roney2022evidence}. However, AF2 structures may contain protein segments that are placed with uncertainty~\citep{akdel2022structural} that need manual inspection instead of purely relying on machines. Most native proteins folded into stable conformations with the lowest free energy~\citep{AnfinsenCb1975ExperimentalAT}. Therefore, both
Atom Transformer~\citep{YilunDu2020EnergybasedMF} and GraphEBM~\citep{DeqinLiu2022SE3EG} are the energy-based models for protein side-chain conformation with different networks, a transformer model and a GNN~\citep{SoumyaSanyal2020ProteinGCNPM, busbridge2019relational} enhanced model, which predicted scores of side-chain conformations for given structures.

Based on AlphaFold-Multimer, ColAttn~\citep{BoChen2022ImproveTP} made use of pLMs to identify interologs of a complex by estimating the column attention weight matrix. \cite{ArneElofsson2022PredictingTS} completed a large protein complex assembly using a Monte Carlo tree search to address the problem of AlphaFold-multimer, whose performance declined rapidly for proteins with three or more chains. Colossal-AI~\citep{bian2021colossal} team has developed pipelines (xTrimoMultimer, xTrimoABFold and xTrimoDock) based on pLMs for the structure prediction of protein complexes and antibodies. To predict the structures of protein-nucleic acid complexes, \cite{MinkyungBaek2022AccuratePO} proposed RoseTTAFoldNA based on RoseTTAFold, which is a unified framework for protein-DNA, protein-RNA complexes, and RNA tertiary structures.

When having a coarse-grained representation of protein structures, EquiFold~\citep{JaeHyeonLee2022EquiFoldPS} predicted protein structures via iterative refinement using an SE(3)-equivariant~\citep{YiLunLiao2022EquiformerEG} neural network. Structure refinement also takes coarse structures as input and output refined coordinates. This process has been integrated into some PSP models, like AF2 and RoseTTaFold. Different from DeepACCNet~\citep{NaozumiHiranuma2020ImprovedPS} and GNNRefine~\citep{XiaoyangJing2021FastAE}, which used predicted distances to guide PyRosetta~\citep{SidharthaChaudhury2010PyRosettaAS} protein structure refinement, a SE(3)-equivariant graph transformer network that is equivariant to the rotation and translation of coordinates was developed in ATOMRefine~\citep{TianqiWu2022AtomicPS} for all-atom structural refinement end-to-end, where initial structures were generated by AF2. In contrast, GNNRefine performs relatively poorly on AF2 structures. Researchers have become adept at working out more challenging problems. For example, DCGAN~\citep{NamrataAnand2018GenerativeMF} has applied generative adversarial networks (GANs) to generate pairwise distance maps from corrupted protein structures and thus recover robust 3D structures.  \cite{KevinEWu2022ProteinSG} trained a denoising diffusion-based generative model with only a vanilla transformer, which generated high-quality, and diverse protein structures inspired by the huge success of diffusion models in a wide range of data modalities~\citep{RobinRombach2022HighResolutionIS, SimonRouard2021CRASHRA}, such kind of generative models can benefit structure refinement, protein conformation and structure prediction by generating biologically plausible and robust structures, it is worth to expect more successes achieved by diffusion model in the biomedical field.

\begin{table*}[t]
	\caption{Representative methods for PSP and related tasks.}
	\label{Table_PSP}
	\setlength{\tabcolsep}{2.8pt}
	\centering
	\small
	\begin{adjustbox}{max width=\linewidth}
		\begin{threeparttable} %
			\begin{tabular}{llllllll}
				\toprule 
				Model &  Evolution  & Energy  & Main Network & Task \\
				\hline 
				\href{https://github.com/aqlaboratory/rgn}{RGN}~\citep{MohammedAlQuraishi2018EndtoEndDL} & \Checkmark & \XSolidBrush & LSTM & PSP \\
				\multirow{2}{*}{\cite{AlbertCosta2021DistillationOM}} & \multirow{2}{*}{\Checkmark} & \multirow{2}{*}{\XSolidBrush} & MSA Transformer & \multirow{2}{*}{PSP}\\
				& & & Graph Transformer~\citep{YunshengShi2020MaskedLP} & \\
				
				\href{https://github.com/deepmind/alphafold}{AF2}~\citep{JohnMJumper2021HighlyAP} & \Checkmark & \XSolidBrush & Evoformer, IPA & PSP \\
				\multirow{2}{*}{\href{https://github.com/RosettaCommons/RoseTTAFold}{RoseTTAFold}~\citep{MinkyungBaek2021AccuratePO}} & \multirow{2}{*}{\Checkmark} & \multirow{2}{*}{\XSolidBrush} &  Graph Transformer & \multirow{2}{*}{PSP} \\
				& & & SE(3)-Transformer~\citep{FabianBFuchs2020SE3Transformers3R} & \\
				
				\href{https://github.com/hpcaitech/FastFold}{FastFold}~\citep{ShengganCheng2022FastFoldRA} & \Checkmark & \XSolidBrush & AF2 & PSP \\
				\href{https://github.com/sokrypton/ColabFold}{ColabFold}~\citep{mirdita2022colabfold} & \Checkmark & \XSolidBrush & AF2 & PSP \\
				\href{https://github.com/PaddlePaddle/PaddleHelix/tree/dev/apps/protein_folding/helixfold}{HelixFold}~\citep{GuoxiaWang2022HelixFoldAE} & \Checkmark & \XSolidBrush & AF2 & PSP \\
				\href{https://gitee.com/mindspore/mindscience/tree/master/MindSPONGE/applications/MEGAProtein}{MEGA-Fold}~\citep{SiruiLiu2022PSPMP} & \Checkmark & \XSolidBrush & AF2 & PSP \\
				\href{https://github.com/dptech-corp/Uni-Fold}{Uni-Fold}~\citep{ZiyaoLi2022UniFoldAO} & \Checkmark & \XSolidBrush & AF2 & PSP \\
				
				EvoGen~\citep{JunZhang2022FewShotLO} & \Checkmark & \XSolidBrush & Attention & MSA Generation \\
				
				\href{https://github.com/facebookresearch/esm}{ESMFold}~\citep{ZemingLin2022LanguageMO} & \XSolidBrush & \XSolidBrush &ESM-2 & Single Sequence PSP \\  
				\href{https://github.com/HeliXonProtein/OmegaFold}{OmegaFold}~\citep{RuidongWu2022HighresolutionDN} & \XSolidBrush & \XSolidBrush & OmegaPLM, Geoformer & Single Sequence PSP \\
				\href{https://github.com/PaddlePaddle/PaddleHelix/tree/dev/apps/protein_folding/helixfold-single}{HelixFold-Single}~\citep{XiaominFang2022HelixFoldSingleMP} & \XSolidBrush & \XSolidBrush & AF2 & Single Sequence PSP\\
				\href{https://github.com/aqlaboratory/rgn2}{RGN2}~\citep{RatulChowdhury2021SinglesequencePS} & \XSolidBrush & \XSolidBrush & AminoBERT & Single Sequence PSP \\
				
				trRosettaX-Single~\citep{WenkaiWang2022SinglesequencePS} & \XSolidBrush & \Checkmark & s-ESM-1b, $\text{Res2Net\_Single}$ & Single Sequence PSP\\
				EquiFold~\citep{JaeHyeonLee2022EquiFoldPS} & \XSolidBrush & \XSolidBrush & SE(3)-Transformer & Antibody Structure Prediciton \\
				
				\href{https://github.com/Graylab/IgFold}{IgFold}~\citep{JeffreyARuffolo2022FastAA} & \XSolidBrush & \XSolidBrush & Graph Transformer, AntiBERTy, IPA & Antibody Structure Prediciton \\
				
				
				\href{https://github.com/deepmind/alphafold}{AlphaFold-Multimer}~\citep{RichardEvans2021ProteinCP} & \Checkmark & \XSolidBrush & AF2 & Complex Structure Prediciton \\
				\cite{PatrickBryant2021ImprovedPO} & \Checkmark & \XSolidBrush & AF2 & Complex Structure Prediciton\\
				
				ColAttn~\citep{BoChen2022ImproveTP}	& \Checkmark & \XSolidBrush & MSA Transformer, AlphaFold-Multimer & Complex Structure Prediciton\\
				
				\cite{ArneElofsson2022PredictingTS} & \Checkmark & \XSolidBrush & AlphaFold-Multimer & Complex Structure Prediciton \\
				
				\multirow{2}{*}{\href{https://github.com/uw-ipd/RoseTTAFold2NA}{RoseTTAFoldNA}~\citep{MinkyungBaek2022AccuratePO}} & \multirow{2}{*}{\Checkmark} & \multirow{2}{*}{\XSolidBrush} & \multirow{2}{*}{RoseTTAFold} & Structure Prediction of RNA, Protein \\
				& & & &-DNA $\&$ Protein-RNA Complexes \\
				\href{https://github.com/RFOLD/RhoFold}{E2Efold-3D}~\citep{TaoShen2022E2Efold3DED} &  \checkmark & \XSolidBrush & Transformer, IPA & RNA Structure Prediction \\
				
				DCGAN~\citep{NamrataAnand2018GenerativeMF} & \XSolidBrush & \checkmark & GAN & Structure Generation\\
				\cite{KevinEWu2022ProteinSG} & \XSolidBrush & \XSolidBrush & Transformer & Structure Generation\\
				
				\href{https://github.com/facebookresearch/protein-ebm}{Atom Transformer}~\citep{YilunDu2020EnergybasedMF} & \XSolidBrush & \Checkmark & Transformer & Protein Conformation\\
				\href{https://github.com/RSvan/SPEACH_AF}{$\text{SPEACH\_AF}$}~\citep{RichardAStein2022SPEACH} & \Checkmark & \XSolidBrush & AF2 & Protein Conformation \\
				GraphEBM~\citep{DeqinLiu2022SE3EG} & \XSolidBrush & \Checkmark & DimeNet~\citep{JohannesKlicpera2020DirectionalMP} & Protein Conformation \\
				
				\href{https://codeocean.com/capsule/5769140/tree/v1}{GNNRefine}~\citep{XiaoyangJing2021FastAE} & \XSolidBrush & \XSolidBrush & GNN & Structure Refinement \\
				ATOMRefine~\citep{TianqiWu2022AtomicPS} & \XSolidBrush & \XSolidBrush & SE(3) Graph Transformer & Structure Refinement \\
				
				\toprule
			\end{tabular}
			\begin{tablenotes} %
				\item \Checkmark and \XSolidBrush appeared in the column of Evolution, and Energy represents this model whether used this information or not. The model name with colour is linked with codes or its server page. Most of these present methods are pLM-aware models. $\&$: and.
			\end{tablenotes} %
		\end{threeparttable}
	\end{adjustbox}
\end{table*}

\section{Discussion: Limitations and Future Trends}
With the million-level protein sequence databases, pLMs have been becoming larger and larger (billion-level parameters for ESM-2), which are dominated by big companies in reality. For example, DeepMind used 128 TPU v3 cores to train and fine-tune AF2 over one week. Training such deep learning models might only be accessible to large companies such as Google; it seems hard for academic research groups to learn protein embeddings from the start, which is also a burden for the theme of a green environment. Considering this problem, researchers can put more attention to methods' innovations. 

Firstly, why not better utilize these large-scale pre-trained pLMs? How to best leverage them is still under-explored compared to pre-trained language models in NLP; it means developing suitable and special transfer learning methods to adapt knowledge to various downstream tasks. Knowledge distillation is inspiring; MSA, structure and function information can be distilled and transferred~\citep{AlbertCosta2021DistillationOM}, which is used in NLP~\citep{ZiqingYang2020TextBrewerAO}. Secondly, a large-scale pLM cannot tackle all problems, e.g., some reports have indicated that AF2 does not appear to be well suited to predict the impact of mutations on proteins~\citep{MarinaAPak2021UsingAT, GwenRBuel2022CanAP}. Structure-triggered tasks cannot be directly transferred to other prediction tasks~\citep{MingyangHu2022ExploringE}. Furthermore, \cite{ErikNijkamp2022ProGen2ET} found bigger models may not translate into better zero-shot fitness performance. Therefore, there still exists space for different models to tackle various problems. Thirdly, ESM-2 concluded that the improvement of low-scale models is easily saturated with high evolutionary depth, while with the low evolutionary depth, it continues when models' sizes increase, which illustrates that combining extra information suitably, including injecting biological and physical priors, using evolutionary information, different levels of structures, GO, etc., can reduce models' size and boost their performance. These different types of information (heterogeneous data) are involved with data mining and task design. Thus, multi-task or multi-modal learning is a direction that deserves to have more exploration~\citep{TristanBepler2021LearningTP}. Finally, since sequence mutations can cause genetic diseases, their effects on function form a landscape that reveals how function constrains sequence. Predicting robust protein structures and understanding the functional effects of sequence mutations are critical. 

The architectures of most current pLMs are the same as LMs' in NLP, i.e., people use these LMs in the protein communities without much adaptation and modification, which hinders the development of pLMs and the understanding of protein grammars. Techniques present in LMs are also used in pLMs, like masking strategies. Proteins and Languages have similarities, but they are not the same as we have mentioned in Section~\ref{Protein and Language}. Therefore, designing proper pLMs and developing suitable methods for protein data considering its properties is an important and urgent problem. 

Despite the proliferation of LMs, these pLM-based models still lack interpretability, hindering people from understanding the mechanism behind protein folding. AF2-like models cannot provide the detailed understanding of molecular and chemical interactions that is important for studies of molecular mechanisms and structure-based drug design. Thus, model interpretability helps researchers find protein grammars useful in biomedical applications. Visualization is a tool that can record the process of protein folding or how the protein functions during various activities. Therefore, developing a high-quality protein tokenization method or combining it with other machine learning methods is appealing, like Bayesian modelling, Monte Carlo strategy, energy functioning, Markov random field, direct coupling analysis~\citep{MartinWeigt2009IdentificationOD}, or diffusion models. 

Due to the different large databases of proteins, people need to be concerned about the wrong information in the databases. Some research groups choose to build new datasets to satisfy their unique needs; data leakage, bias, and ethics should be considered in this situation. For instance, ProteinKG25 was created for utilizing protein sequence and functions~\citep{NingyuZhang2022OntoProteinPP} better to get meaningful embeddings. On the other hand, building complete, reliable, and just benchmarks is essential to evaluating various models and promoting the appearance of solid methods.

Scientists have been developing a unified model for DNA, RNA, and protein engineering in the biomedical domain~\citep{BenyouWang2022PretrainedLM}, BERT-RBP~\citep{KeisukeYamada2021PredictionOR} adopted BERT architecture to predict RNA-protein interactions, still has a distance to go to interpret their relationships well. Single protein sequences, protein-ligand complexes, and RNA complexes structure prediction and conformation modelling have been appealing to a group of researchers. These problems are more complicated than those in PSP, and they are not yet solved. Even for PSP, there is still space for models predicting structures with ultra-high accuracy (resolution less than $0.5\AA$).

\section{Databases}
\label{Databases}
We follow the mapping for LMs from NLP to proteins in ProtTrans~\citep{AhmedElnaggar2022ProtTransTC}, which interpret proteins as "sentences". Therefore, the number of proteins that needed disk space for datasets and official web pages are listed in Table~\ref{datasets}. 

In detail, UniProt~\citep{2012UpdateOA} provides a comprehensive, high-quality, and freely accessible resource of protein information, where UniProt databases include UniProtKB, UniRef~\citep{BarisESuzek2015UniRefCA}, UniPac databases. The UniProt Knowledgebase (UniProtKB) is comprised of two sections, UniProtKB/Swiss-Prot and UniProtKB/TrEMBL. The former provides the reviewed relevant information about a particular protein, including protein and gene names, function, protein-protein interactions, etc. Proteins in the latter largely have no experimental data available, while these unreviewed records are enriched with automatic annotation and classification. The UniRef databases (UniProt Reference Clusters) ~\citep{BarisESuzek2015UniRefCA} provide clustered sets of sequences from the UniProt Knowledgebase (UniProtKB) and provide complete coverage of sequence space at several resolutions (100$\%$, 90$\%$, 50$\%$ identity) in a hierarchical fashion. UniRef50 clusters are generated using UniRef90 clusters, which are based on UniRef100 clusters. UniRef databases have a broad range of usages, like functional annotation, family classification, systems biology, structural genomics, phylogenetic analysis, and mass spectrometry. The UniProt Archive (UniParc) is the most comprehensive publicly accessible non-redundant protein sequence database without record annotation.

The Protein Data Bank (PDB)~\citep{wwpdb2019protein} is a database for the experimentally determined three-dimensional structural data of biological macromolecules, including the sequence and 3D structures of proteins. The number of structures in the PDB has grown at an approximately exponential rate based on historical experience, and there are 170k multi-chain protein structure files as of October 2021. However, a million-level protein structure prediction named as PSP~\citep{SiruiLiu2022PSPMP} was presented based on PDB after the appearance of AF2 with 570k true structure sequences and 745k complementary distillation sequences. 

The CATH~\citep{ChristineAOrengo1997CATHA} is a novel public hierarchical classification database of protein domain structures for public download, where these domains are obtained from protein three-dimensional structures deposited in the PDB. The domains are classified into four main levels: protein class (C), which describes the secondary structure composition of each domain, i.e., all alpha, all beta, mixed alpha-beta, or few secondary structures; at the architecture (A) level, the arrangement of secondary structures is summarized; at the topology/fold (T) level, the sequential connectivity is taken into account; at the homologous superfamily (H) level, proteins have a demonstrable evolutionary relationship. Structured Transformer~\citep{JohnIngraham2019GenerativeMF} uses CATH4.2, processed and cluster-split into training, validation, and test sets, which contain 18025 chains in the training set, 1637 chains in the validation set, and 1911 chains in the test set. The latest release of CATH-Gene3D (v4.3) has 151 million protein domains classified into 5,841 superfamilies and is to predict the locations of structural domains on millions of publicly available protein sequences. 

The Big Fantastic Database (BFD) is a sequence profile database and is one of the largest metagenomic databases, as it keeps one copy of duplicates from UniProt and other big protein databases. These sequences were clustered by a sequence identity cut-off of 30$\%$ and a coverage threshold of 90$\%$ using MMseqs2/Linclust~\citep{MartinSteinegger2018ClusteringHP, MartinSteinegger2019ProteinlevelAI, HOU2022434}, e.g., the BFD30 dataset was clustered to 65 million clusters at 30$\%$ sequence identity. Searching for a protein against BFD is slow but more sensitive. Sometimes it is convenient to use MSA, computed from each of the BFD clusters.

Pfam~\citep{SaraElGebali2019ThePP} is a database of protein families used extensively in bioinformatics. It aims to provide a complete and accurate classification of protein families and domains, which includes annotations and alignments generated by hidden Markov models (HMMs). \textit{pfamseq} is a profile HMM that is queried against a sequence database based on UniProtKB and used to find homologues for a Pfam entry. The recent version of Pfam contains 19,632 families; each family includes descriptions, alignments, architectures, etc.

The AlphaFold Protein Structure Database (AlphaFoldDB) is a collection of protein structure predictions created by DeepMind in partnership with EMBL-EBI. These 3D structures are predicted by AlphaFold, which achieves accuracy competitive with experiments. The latest database release contains over 200 million entries for UniProt.

ProteinKG25 is a large-scale Knowledge Graph (KG) dataset with aligned descriptions and protein sequences, respectively, to Gene Ontology (GO) terms and protein entities~\citep{NingyuZhang2022OntoProteinPP}. Go terms are seen as graph nodes, and the relationships between the terms are edges. ProteinKG25 combines these two different structures, GO and Gene Annotation into a unified KG for training LMS that incorporates GO information. It includes most of the triplets (Protein-GO triplets and GO-GO triplets) and a few entities (proteins and gene terms) and relations.

Uniclust databases~\citep{MilotMirdita2017UniclustDO} cluster UniProtKB sequences at the level of 90$\%$, 50$\%$ and 30$\%$ pairwise sequence identity, formed Uniclust90, Uniclust50, Uniclust30. Compared with UniRef, which relied on the CD-HIT software for clustering, Uniclust databases used the developed software suite MMseqs2, which had higher consistency in the functional annotation. Furthermore, Uniclust sequences are annotated with matches to other commonly used datasets (Pfam, SCOP~\citep{TimHubbard1997SCOPAS} and PDB), which may not be annotated in UniProt with HHblits~\citep{MartinSteinegger2019HHsuite3FF}.

The Structural Classification of Proteins (SCOP) database~\citep{TimHubbard1997SCOPAS} was created by manual classification of protein structural domains based on similarities of their structures and evolutionary relationships. Similar to CATH and Pfam, the original hierarchical organizations of SCOP are class, fold, superfamily, and family. The new version, SCOP2, was released in 2020 to provide a better database for protein structure annotation and classification. Structural Classification of Proteins—extended (SCOPe) extends the SCOP database of protein structural relationships. The ASTRAL compendium provides tools to help research protein structure and evolution. The SCOPe has corrected errors in SCOP and incorporated the Astral database~\citep{JohnMarcChandonia2017SCOPeMC}. The latest release of SCOPe ASTRAL 2.08 has more than 50K protein sequences with known structures and SCOP classifications.

Critical Assessment of Protein Structure Prediction (CASP) is a worldwide experiment for PSP that will have been conducted 15 times by the end of 2022. Research groups from all over the world participate in CASP to objectively test their structure prediction methods. By categorizing different themes, like quality assessment, model refinement, domain boundary prediction, protein complex structure prediction, etc., and selecting target proteins, CASP researchers can identify what progress has been made and highlight the future efforts that may be most productively focused on.


\begin{table*}[t]
	\caption{Information of Protein Databases}
	\label{datasets}
	\setlength{\tabcolsep}{2.8pt}
	\centering
	\small
	\begin{adjustbox}{max width=\linewidth}
		\begin{threeparttable} %
			\begin{tabular}{llllllll}
				\toprule 
				Dataset & $\#$Proteins & Disk Space & Description & Link \\
				\hline 
				UniProtKB/Swiss-Prot & 500K & 0.59GB& knowledgebase & \url{https://www.uniprot.org/uniprotkb?query=*} \\
				UniProtKB/TrEMBL & 229M & 146GB & knowledgebase & \url{https://www.uniprot.org/uniprotkb?query=*} \\
				UniRef100 & 314M &76.9GB & clustered sets of sequences & \url{https://www.uniprot.org/uniref?query=*}  \\
				UniRef90 & 150M  & 34GB & 90$\%$ identity & \url{https://www.uniprot.org/uniref?query=*}\\
				UniRef50 & 53M &  10.3GB & 50$\%$ identity & \url{https://www.uniprot.org/uniref?query=*}\\
				UniParc & 528M  & 106GB & Sequence & \url{https://www.uniprot.org/uniparc?query=*}\\
				PDB & 190K & 50GB & 3D structure & \url{https://www.wwpdb.org/ftp/pdb-ftp-sites}\\
				CATH4.3 & N/A & 1073MB & hierarchical classification & \url{https://www.cathdb.info/} \\
				BFD & 2500M & 272GB & sequence profile & \url{https://bfd.mmseqs.com/} \\
				Pfam & 47M & 14.1GB & protein families &\url{https://www.ebi.ac.uk/interpro/entry/pfam/} \\
				AlphaFoldDB & 214M & 23 TB & predicted 3D structures &\url{https://alphafold.ebi.ac.uk/} \\
				ProteinKG25 & 5.6M & 147MB & a KG dataset with GO & \url{https://drive.google.com/file/d/1iTC2-zbvYZCDhWM_wxRufCvV6vvPk8HR} \\
				Uniclust30 & N/A & 6.6GB & clustered protein sequences & \url{https://uniclust.mmseqs.com/} \\
				SCOP & N/A & N/A & structural classification & \url{http://scop.mrc-lmb.cam.ac.uk/} \\
				SCOPe & N/A & 86MB & extented version of SCOP & \url{http://scop.berkeley.edu}\\
				
				\toprule
			\end{tabular}
			\begin{tablenotes} %
				\item K, thousand; M, million, disk space is in GB or TB (compressed storage as text), which is estimated data influenced by the compressed format.
			\end{tablenotes} %
		\end{threeparttable}
	\end{adjustbox}
\end{table*}

\section{Conclusion}
This paper systematically summarizes recent advances in pLMs, PSP, and related tasks, including background, why and how pLMs are used in protein representation learning, existing pLMs and PSP methods, the relationships between pLMs and PSP, and how pLMs function in the development of protein folding. A set of databases are introduced. Furthermore, we also discuss some limitations, possible tackling directions, and future trends. Finally, we expect that LMs and pLMs can aid more in the specific biochemical, biomedical, and bioinformatic domains.


==> sec5_4_OpportunitiesChallenges.tex <==
\subsubsection{Challenges}




\subsubsection{Opportunities of Diffusion-Based and Flow-Based Models for Tree Generation}

Recently, diffusion-based and flow-based models have emerged as powerful generative models for a wide range of applications, including image generation, text synthesis, and molecular design. These models have unique properties that could be harnessed for tree generation, providing new directions for research in this area.

\textbf{Diffusion-Based Models} such as Denoising Diffusion Probabilistic Models (DDPMs) have demonstrated remarkable success in generating high-quality samples through a progressive denoising process. Integrating diffusion models with tree structures, as seen in \textbf{Diffuse-TreeVAE}, shows promise for generating hierarchical and tree-like data representations \cite{goncalves_structured_2024}. By utilizing a latent tree structure to guide the diffusion process, these models can potentially generate more coherent and structured tree samples that adhere to predefined constraints such as acyclicity and hierarchy. The integration of DDPMs with tree generation tasks could lead to better sample diversity and quality, overcoming some of the limitations of previous VAE-based approaches.

\textbf{Flow-Based Models} like Normalizing Flows are another promising direction for tree generation. Flow-based models use invertible transformations to map complex distributions to simpler ones, allowing for exact likelihood computation and efficient sampling. When adapted for tree generation, flow-based models could leverage hierarchical latent variable models to represent tree structures in a more flexible and tractable way. By combining normalizing flows with tree-based priors, it is possible to create generative models that capture both the local dependencies (e.g., parent-child relationships in trees) and global properties (e.g., overall tree structure) effectively. Future work could explore the use of \textbf{hierarchical normalizing flows} for generating large and complex tree structures, particularly for applications in phylogenetic analysis and hierarchical clustering.

Overall, diffusion-based and flow-based models present a promising frontier for tree generation tasks. By leveraging the strengths of these models in handling complex distributions and their potential for scalability and flexibility, researchers can develop more advanced tree generation frameworks that can effectively tackle the challenges of generating large, hierarchical, and highly structured tree-like data.


==> sec6_1_Evolution.tex <==
\subsection{Species Evolution and Gene Evolution Analysis}

Phylogenetic trees serve as a critical analytical tool in evolutionary biology, demonstrating their irreplaceable value in studying evolution across multiple biological scales—from molecules and genes to species. By revealing evolutionary relationships at different levels, phylogenetic trees not only help us understand the origins and processes of life's diversity but also provide a new theoretical framework and research pathways for complex biological phenomena.

\textit{Molecular-Level Evolutionary History:}
At the most fundamental molecular level, molecular phylogenetics uses molecular data (such as DNA, RNA, or protein sequences) to reconstruct and analyze the evolutionary relationships of species or genes. Phylogenetic trees play a crucial role at this level by helping to trace the evolutionary processes of specific genomic features and traits. For example, the study by Marletaz et al. \citep{marletaz_little_2023} used phylogenetic analysis to reveal how genome reorganization and regulatory variation in the little skate (\textit{Leucoraja erinacea}) drive the evolution of new phenotypic traits, such as the wing-like pectoral fins. Similarly, the study on genome evolution in wild and cultivated potatoes \citep{tang_genome_2022} used phylogenetic trees to examine the expansion of disease-resistance genes, shedding light on their evolutionary trajectories under selective pressures. These studies challenge traditional views of phenotypic evolution, suggesting that structural changes in the genome and the reconfiguration of regulatory networks can lead to significant morphological variation, not merely gene mutations. This expands our understanding of phenotypic evolutionary mechanisms and underscores the importance of integrating genomic data with phylogenetic information.

\textit{Evolution of Gene Families and Functional Adaptations:}
At the level of gene families, phylogenetic trees are essential for understanding the expansion and functional adaptation of gene families. For example, the study by Balart-García et al. \citep{balart-garcia_parallel_2023} analyzed parallel and convergent genomic changes in beetles that have adapted to subterranean environments, revealing the critical role of gene family expansions in ecological adaptation. Such studies highlight the role of phylogenetic trees in tracing the history of gene expansion and emphasize their value in understanding how gene functions change under different environmental pressures. Exploring the interplay between gene expansion and environmental adaptation helps uncover the complex dynamics of innovation and selection in evolutionary processes. Integrating phylogenetics with biogeographical data can further explore the historical patterns and distribution of gene expansion and ecological adaptation. For instance, the reclassification of the genus \textit{Capparis} \citep{maurya_molecular_2023} used molecular phylogenetic tools to reveal evolutionary paths in their biogeographical history.

\textit{Lineage-Specific Genomic Evolution:}
At a higher level, phylogenetic trees are used to study the evolutionary pathways of genomes within specific lineages, revealing how genome structures change in response to different lineage pressures. For instance, Bredemeyer et al. \citep{bredemeyer_single-haplotype_2023} investigated structural variations in felid genomes, demonstrating how phylogenetic trees can be used to trace the evolutionary trajectories of these structural variations and their significance in species-specific adaptations. This approach prompts us to rethink the role of genomic structural changes in species divergence and adaptation, viewing them not merely as neutral evolutionary events. By integrating different levels of data, these studies help provide a more comprehensive understanding of the evolutionary paths of species and genes in historical environments.

\textit{Evolutionary Impact of Horizontal Gene Transfer (HGT):}
In the study of horizontal gene transfer (HGT), phylogenetic trees are essential tools for understanding how gene flow influences species evolution. Sahu et al. \citep{sahu_vertical_2023} investigated HGT in the fungal genus \textit{Armillaria}, showing how phylogenetic trees can effectively trace the evolutionary integration of horizontally acquired genes and their impact on pathogenicity and ecological adaptation. This analysis not only reveals potential mechanisms of rapid adaptation to new environments through HGT but also underscores the importance of reevaluating traditional vertical evolution models.

\textit{Macroevolutionary Analysis at the Species Level:}
At the highest level of species evolution, phylogenetic trees are used to uncover macroevolutionary patterns and processes, such as speciation and radiation. Wright et al. \citep{wright_comparative_2024} employed phylogenetic trees to conduct an in-depth analysis of chromosome evolution in Lepidoptera, revealing conserved and dynamic chromosomal rearrangements over 250 million years. Stiller et al. \citep{stiller_complexity_2024} used phylogenetic analysis to resolve the complex evolutionary relationships among avian lineages, providing insights into the rapid radiation of Neoaves. These studies highlight the necessity of phylogenetic analysis at the species level, not only to reveal new evolutionary relationships but also to challenge and revise previous evolutionary hypotheses. Combining molecular phylogenetics with biogeographical analysis can better understand the historical distribution and speciation patterns of species, which is particularly important for interpreting the biogeographical context of species evolution.

\textit{Comprehensive Phylogenetic Analysis with Multi-level Data Integration:}
Comprehensive phylogenetic analyses often require integrating multiple levels of data. For instance, the phylogenetic placement of the sessile euglenid \textit{Dolium sedentarium} \citep{lax_molecular_2023} was resolved using both single-cell transcriptomics and multigene phylogenies. This integrative approach not only clarifies the evolutionary position of unique taxa but also enhances our understanding of broader evolutionary patterns. By incorporating multiple types of data, this method helps reveal the complexity of evolutionary processes and improves the interpretation of biodiversity evolution.


==> tab_classical_biotree.tex <==

\begin{table*}[t]
    \centering
    \footnotesize
    \caption{Summary of Phylogenetic Tree Construction Methods}
    \begin{tabular}{p{2cm}| p{6cm} p{3cm} p{5cm}}
        \toprule
        \textbf{Data Type} & \textbf{Method}                           & \textbf{Method Classification} & \textbf{Publication Year}        \\
        \midrule
        \multirow{9}{*}{\textbf{Sequence}}
                           & UPGMA                                     & Distance Matrix                & \citep{Michener1957}             \\
                           & Neighbor-Joining (NJ)                     & Distance Matrix                & \citep{Saitou1987}               \\
                           & Minimum Evolution (ME)                    & Distance-Based                 & \citep{Rzhetsky1992}             \\
                           & RAxML                                     & Maximum Likelihood             & \citep{Stamatakis2014}           \\
                           & PhyML                                     & Maximum Likelihood             & \citep{Guindon2003}              \\
                           & IQ-TREE                                   & Maximum Likelihood             & \citep{Nguyen2015}               \\
                           & MrBayes                                   & Bayesian Inference             & \citep{Ronquist2012}             \\
                           & BEAST                                     & Bayesian Inference             & \citep{Drummond2012}             \\
                           & Maximum Parsimony (MP)                    & Character-Based                & \citep{Fitch1971}                \\
        \midrule

        \multirow{4}{*}{\textbf{Protein}}
                           & Multiple Sequence Alignment (MSA)         & Sequence-Based                 & \citep{Thompson1994, Edgar2004}  \\
                           & Structural Alignment                      & Structure-Based                & \citep{Holm1993, Zhang2005}      \\
                           & Homology Modeling-Based Phylogeny         & Structure-Based                & \citep{Sali1993}                 \\
                           & Single-Cell Proteomics Analysis           & Single-Modality                & \citep{Wagner2019}               \\
        \midrule

        \multirow{4}{*}{\textbf{RNA-seq}}
                           & Single-Cell RNA-seq (scRNA-seq) Analysis  & Single-Modality                & \citep{Stuart2019, Trapnell2014} \\
                           & Temporal Multi-Omics Analysis             & Multi-Modality                 & \citep{Tran2020}                 \\
                           & Integrated Multi-Omics Analysis           & Multi-Modality                 & \citep{Stuart2019}               \\
                           & Joint Dimensionality Reduction Techniques & Multi-Modality                 & \citep{Argelaguet2020}           \\
        \midrule

        \multirow{2}{*}{\textbf{ATAC-seq}}
                           & Single-Cell ATAC-seq Analysis             & Single-Modality                & \citep{Granja2020}               \\
                           & Temporal Multi-Omics Analysis             & Multi-Modality                 & \citep{Tran2020}                 \\
        \midrule

        \multirow{2}{*}{\textbf{DNA-seq}}
                           & Single-Cell DNA Methylation Analysis      & Single-Modality                & \citep{Clark2017}                \\
                           & Graph-Based Multi-Omics Analysis          & Multi-Modality                 & \citep{Wolf2019}                 \\
        \midrule

        \multirow{2}{*}{\textbf{Multi-Omics}}
                           & Graph-Based Multi-Omics Analysis          & Multi-Modality                 & \citep{Wolf2019}                 \\
                           & SCORPIUS                                  & Multi-Modality                 & \citep{Cannoodt2016}             \\
        \bottomrule
    \end{tabular}
    \label{tab:phylogenetic_methods_summary}
\end{table*}

